Estimating the Longest Increasing Subsequence in Nearly Optimal Time

Longest Increasing Subsequence (LIS) is a fundamental statistic of a sequence, and has been studied for decades. While the LIS of a sequence of length $n$ can be computed exactly in time $O(n\log n)$, the complexity of estimating the (length of the) LIS in sublinear time, especially when LIS $\ll n$, is still open. We show that for any integer $n$ and any $\lambda = o(1)$, there exists a (randomized) non-adaptive algorithm that, given a sequence of length $n$ with LIS $\ge \lambda n$, approximates the LIS up to a factor of $1/\lambda^{o(1)}$ in $n^{o(1)} / \lambda$ time. Our algorithm improves upon prior work substantially in terms of both approximation and run-time: (i) we provide the first sub-polynomial approximation for LIS in sub-linear time; and (ii) our run-time complexity essentially matches the trivial sample complexity lower bound of $\Omega(1/\lambda)$, which is required to obtain any non-trivial approximation of the LIS. As part of our solution, we develop two novel ideas which may be of independent interest: First, we define a new Genuine-LIS problem, where each sequence element may either be genuine or corrupted. In this model, the user receives unrestricted access to actual sequence, but does not know apriori which elements are genuine. The goal is to estimate the LIS using genuine elements only, with the minimal number of "genuiness tests". The second idea, Precision Forest, enables accurate estimations for composition of general functions from "coarse" (sub-)estimates. Precision Forest essentially generalizes classical precision sampling, which works only for summations. As a central tool, the Precision Forest is initially pre-processed on a set of samples, which thereafter is repeatedly reused by multiple sub-parts of the algorithm, improving their amortized complexity.

==> abstract_text.tex <==
Longest Increasing Subsequence (LIS) is a fundamental statistic of a sequence, and has been studied for decades. While the LIS of a sequence of length $n$ can be computed exactly in time $O(n\log n)$, the complexity of estimating the (length of the) LIS in sublinear time, especially when LIS $\ll n$, is still open.

We show that for any $n \in \N$ and $\lambda = o(1)$, there exists a (randomized) \emph{non-adaptive} algorithm that, given a sequence of length $n$ with LIS $\ge \lambda n$, approximates the LIS up to a factor of $1/\lambda^{o(1)}$ in $n^{o(1)} / \lambda$ time. Our algorithm improves upon prior work substantially in terms of both approximation and run-time: (i) we provide the first sub-polynomial approximation for LIS in sub-linear time; and (ii) our \emph{run-time complexity} essentially matches the trivial \emph{sample complexity} lower bound of $\Omega(1/\lambda)$, which is required to obtain any non-trivial approximation of the LIS.

As part of our solution, we develop two novel ideas which may be of independent interest. First, we define a new Genuine-LIS problem, in which each sequence element may be either genuine or corrupted. In this model, the user receives unrestricted access to the actual sequence, but does not know a priori which elements are genuine. The goal is to estimate the LIS using genuine elements only, with the minimal number of tests for genuineness. The second idea, {\em Precision Tree}, enables accurate estimations for compositions of general functions from ``coarse'' (sub-)estimates. {\em Precision Tree} essentially generalizes classical precision sampling, which works only for summations. As a central tool, the {\em Precision Tree} is pre-processed on a set of samples, which thereafter is repeatedly used by multiple components of the algorithm, improving their amortized complexity.

==> amended_old.tex <==
\newpage

\ns{From now on should be omitted!!}


\section{Old stuff: Algorithm for $\reslis$, proof of Theorem~\ref{thm::sl_rec} - amended}

To bypass the issue, we introduce some more definitions.

\paragraph{Tree notation.}
Assume $b/n^\eps$ is some power of 2 (otherwise, pad it on the right with at most twice as many samples). For $t \in [n^\eps]$, let $T_t = (V_t, E_t)$ be a binary tree\snote{Complete binary tree, i.e., all possible edges present?} of height $\log_2 1/\lambda$ and let \blue{$T = (V,E)$, where $V = \cup_t V_t$ and $E = \cup_t E_t$, }%$T = (\cup_t V_t,\cup_t E_t)$
be a forest. Each node $v^r_{i}$ represent a $(r,i)$ pair with $r \in 2^{[\log_2 1/\lambda]}$ and $i \in [r]$. \blue{For a node $v=v^r_i$, we use $r_v$ to denote $r$, the length of the interval corresponding to $v$.}\snote{Added this definition because I couldn't find it anywhere.}%n interval $X_i^r$. The leaves $v^1_i$ represent the smallest-size intervals $X_i^1$, and each node $v^r_i$ represent interval $X^r_{i}$.

%To make it a tree, we assign to 
Each $v_i^r$ is assigned with following children:\snote{Let's use something like $\mathsf{left}$ and $\mathsf{right}$ for left and right children respectively. It's getting really confusing with $r$ also denoting the radius.}
$$l(v_i^r) \triangleq v_{2i-1}^{r/2}
\hspace{10mm}
r(v_i^r) \triangleq v_{2i}^{r/2}$$

% Note that each node represent a concatenation of both children. 

The root of each tree is $v_t^{1/\lambda}$.

We use the following notation on each node $v \in V_t$: 

First, $X_v$ is an $X_i^r$ interval and $\cY_v \triangleq Y^r_{i,*}$ is the set of candidate intervals.

%For $\Yleft$ and $\Yright$ intervals, we first 

For the next notations, we introduce the following definition.

\begin{definition}
	Fix a set of non-overlapping intervals $S \subseteq \cI$ and an interval $I \in \cI$. Define the {\em containing} interval $\cont(I,S)$ to be the interval $J \in S$ with $I \subseteq J$ if such exists and $\bot$ otherwise.
\end{definition}

For each candidate interval $Y_{v,j} \in \cY_v$, we define the left extension and right extension, respectively, as follows: $\Yleft_{v,j} \triangleq [0, \max Y_{v,j}] \cap \cont(Y_{v,j},\cY_{l(v)})$ and $\Yright_{v,j} \triangleq [\min Y_{v,j},\infty] \cap \cont(Y_{v,j},\cY_{r(v)})$. Define the 2-side extension $\Yboth_{v,j} \triangleq \Yleft_{v,j} \cup \Yright_{v,j}$.

Sometimes, we use the shorthand $\Yleft$, $\Yright$ and $\Yboth$ when the node $v$ is clear from context.

Let $\cYleft_v$, $\cYright_v$ and $\cYboth_v$ the set of all such $\Yleft$, $\Yright$ and $\Yboth$ for a node $v$ (noting that, unlike $\cY_v$, such extensions can actually be overlapping).


%We also index the nodes at each level:

%$$V^r \triangleq [v^r_i]_{i \in [b/r]}$$

\ns{Below to be omitted. we just keep the below until we clean things up...}


\paragraph{Previous notation.}
Define the left child and right child of interval $X_i^r$, respectively, as follows: $l(X_i^r) \triangleq X_{2i-1}^{r/2}$ and $r(X_i^r) \triangleq X_{2i}^{r/2}$.

%For $y$-intervals, we first introduce the following definition.

%\begin{definition}
%	Fix a set of non-overlapping intervals $S \subseteq \cI$ and an interval %$I \in \cI$. Define the {\em containing} interval $\cont(I,S)$ to be the %interval $J \in S$ with $I \subseteq J$ if such exists and $\bot$ %otherwise.
%\end{definition}

For each candidate interval $Y^r_{i,j}$, we define the left child and right child, respectively, as follows: $L_{i,j}^r \triangleq [0, \max Y_{i,j}^r] \cap \cont(Y_{i,j},Y^{r/2}_{2i-1,*})$ and $R_{i,j}^r \triangleq [\min Y_{i,j}^r,\infty] \cap \cont(Y^r_{i,j},Y^{r/2}_{2i-1,*})$.

\paragraph{Algorithm:}
Finally, our algorithm proceeds as follows:

%We observe that \Cref{thm:main} follows from \Cref{thm:technical}. To see this, we call \ALG with input $X=[n],Y=\N$, the input sequence $y$, and $\lambda$, where $\LIS(X,Y)=\lambda n$, and then scale the output $\textsf{out}$ of \ALG suitably.

\begin{figure}[t] \label{fig::ALG_reslis_new}
\setstretch{1.2}
  \begin{algorithm}[H]
    \caption{\reslis}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{intervals $X, Y \subset \N$, a string $y \in \N^{|X|}$, block size $b$ %(assume for now an interval\ns{we expect most blocks LIS to intersect with ``one part'' of $Y$ and in any case should be easily reducible to that})
and parameter $\lambda \in (1/n,1)$.}
		\KwOut{A number $\widehat{\Lambda} \in \left[\LIS(X,Y) \cdot \lambda^{o(1) }- \lambda |y \cap Y|, \LIS(X,Y) \right]$.%\snote{Does this mean $1/\lambda^{o(1)}$?}\nnote{Yes!}
		}
		
		Set $b \gets n^\eps / \lambda$.\\ %\ns{I think $b = n^\eps$ suffices.} 
   % and $t \gets O_\epsilon(\polylog(1/\lambda)/\lambda)$.\\
    If $|X| < b \log n$\snote{Should this be $|X \cap Y^{-1}| < b \log n$? How do we handle the case when $|X| > b \log n$ but $|X \cap Y^{-1}| < b \log n$?}, compute and return $\widehat{L}=\LIS(X,Y)$ exactly.\\
    Otherwise, sample $s= b \cdot \log n$ elements $(w_1, y_{w_1}), (w_2, y_{w_2}), \cdots, (w_s, y_{w_s})$  %$x$-coordinates 
    uniformly from $X \cap Y^{-1}$ by {\em rejection sampling}, where $w_1 < w_2 < \cdots < w_s$. \blue{For convenience, we define $w_0 = 0$.}\\ 
        \For{$r \in 2^{[\log_2 1/\lambda]}$}{
     Let $X^r_1,\ldots,X^r_{b/r}$ be a partition of $X$ into $b/r$ consecutive disjoint intervals each consisting of $r\cdot \log n$ (non-rejected) samples, i.e., $X^r_i = (w_{(i-1)r\log n}, w_{ir\log n}]$.\footnote{Note that we do not impose that $X_i$'s have equal width.}  \\
     For $i \in [b/r]$, let $\cS^r_i=(y_{((i-1)r+j)\log n})_{j\in[r]}$ be the $y$ values of the $r$ samples in $X^r_i$ whose order is a multiple of $\log n$, sorted in descending order. For $j \in [r-1]$, define %; %We assume (by construction) such $\cS^r_i$ are in decreasing order;
     %Let $\{Y^r_{i,j}\}_{j\in [r-1]} \triangleq 
     $Y^r_{i,j} \triangleq [\cS^r_i(j+1),\cS^r_i(j)]$\snote{Should one of the interval end points be excluded? Also, changed the wording slightly.}, and let $Y^r_{i,j}$ be the candidate intervals for block $i$ (again, in descending order).\nnote{we used decreased order to ``force'' the longest $\genlis$ having at most one $j$ for each $i$} \\
      \For{$k \in 2^{[\log_2 1/\lambda]}$}{
  %     Let $g \triangleq Y_{1,1},Y_{1,2},\ldots,Y_{1,r-1},Y_{2,1},\ldots,Y_{b/r,r-1}$ be a $\genlis_b$ input string.  \\
       Let $g_{r,k} \triangleq [(\Yboth_{v_i^r,j} \nnote{this is abuse of notation since $\genlis$ is defined on numbers and not intervals. I will see if I can reduce to fixed numbers and if not, will define inputs for both $\genlis$ and $\reslis$ to be of interval spaces to avoid such an issue. in any case dont expect an issue here...},\1[\reslis(l(X_{v_i^r}),\Yleft_{v_i^r,j},\tfrac{1}{k}) + \reslis(r(X_{v_i^r}),\Yright_{v_i^r,j},\tfrac{1}{k}) > 2\tfrac{|y \cap Y|}{bk}])]_{i \in [b/r],j \in [r-1]}$. \nnote{We first order by $i$, then by $j$. Note that we use interval input rather than numbers for now.}\\
  %     Let $\1[\reslis(X_i,Y_{i,j},1/k) > 1/k]$ be the genuine value of each element of $g$. \\
       Compute $\Lambda_{r,k} \gets \genlis(g_{r,k},k \lambda) \cdot 0.9 \tfrac{|y \cap Y|}{bk}$.\\}}
    Return $\widehat{\Lambda} \gets \max_{r,k} \Lambda_{r,k}$.%\cdot \log^2 1/\lambda$.
\end{algorithm}
\end{figure}


\subsubsection{Analysis}

%We will analyze the lower bound and upper bound of our estimator.
Before analyzing the estimator $\widehat{\Lambda}$, we first prove some essentials invariants of our construction:

\begin{lemma}\label{lm::reslis_invariants_new}
    Fix input $X,Y, y$ to \reslis \blue{, with $|X \cap Y^{-1}| \geq b \log n$.} W.h.p, all the following invariants holds for $\reslis$ algorithm:\snote{Specify the failure probability, say $1-1/n$.}
    \begin{enumerate}
    	\item For all $v \in V$: $|y(X_v) \cap Y| \in [0.9,1.1]\tfrac{r_v |y \cap Y|}{b}$.\snote{Are we explicitly not allowing duplicates? If duplicates are allowed, it could be the case that $|y(X) \cap Y| < |X \cap Y^{-1}|$. Since we are sampling w.r.t $X$, the correct quantity is $|X \cap Y^{-1}|$.}
    	\item For all $v,j$: $|y(X_v) \cap Y_{v,j}| \in [0.9,1.1]\tfrac{|y \cap Y|}{b}$. 
        \item For all $v,j$: $|y(X_v) \cap \Yleft_{v,j}|,|y(X_v) \cap \Yright_{v,j}|  \leq 1.1\tfrac{|y \cap Y|}{b}$. 
    	\item For all $r$ and all sets of pairs $\{(i,\Yboth_{v_i^r,j})\}_i$ that are {\em coherent}, we have $\sum_i \LIS(X_{i},Y^r_{i,j}) \leq \LIS(X,Y)$.
    	\item There exists sets $P_r \subseteq \N \times \cI$ which are {\em coherent} for each $r$, such that %$(i,Y_{i,j}) \in $ that are independently {\em coherent} for each $r$, such that 
    	$$\sum_r \sum_{(i,L^r_{i,j} \cup R^r_{i,j}) \in P_r} \LIS(l(X^r_{i}),L^r_{i,j}) + \LIS(r(X^r_{i}),R^r_{i,j}) \geq \LIS(X,Y) - 2.2\lambda |Y \cap y|.$$
    \end{enumerate}
\end{lemma}

The first 3 invariants are straight-forward, to prove item (4), we add another notation. Fix an optimal $\LIS(X,Y)$ alignment and let $X^*$ be its $x$-coordinates (ie $|X^*| = \LIS(X,Y)$). Define $U_v \subseteq Y$ as the minimal interval containing all $\reslis$ values of $X_v$, ie:
$$U_v \triangleq [\min y(X^* \cap X_v),\max y(X^* \cap X_v)]$$

\begin{fact}
    If $P \subseteq \N \times \cI$ is coherent, then take any $P'$ such that the second coordinates of $P'$ are contained in the second coordinates of $P$. Then $P'$ is coherent.
\end{fact}

%\ns{I think we should define everything on trees $T_t$ as described earlier, and then we use notation of nodes, like $U_v$, $X_v$, $l_v$, $\cY_v$ for the set of $Y_{i,j}^r$, etc...}

%Last, for each $v$, let $Y_v \triangleq \cup_{Y' \in \cY_v: Y' \subseteq U_v} Y'$.

%First, observe the following fact:
%\begin{fact}
%	Fix $r$. (i) $\sum_i \LIS(X_i^r, U_i^r) = \LIS(X,Y)$. (ii) Fix also $i$. %whp: $y(X_i^r) \cap (U_i^r \setminus Y_i^r) \leq 2.2 \tfrac{|y \cap %Y|}{b}$.
%\end{fact}

%\begin{corollary}
%	$\sum_i \LIS(X_i^{1/\lambda}, Y_i^{1/\lambda}) \geq \LIS(X,Y) - %2.2\lambda |y \cap Y|$
%\end{corollary}

We show the following key claim:

\begin{claim}
	    	Fix $v = v_{i'}^{r'}$.  There exists sets $P_r \subseteq \N \times \cI$ which are {\em coherent} for each $r \leq r'$, such that %$(i,Y_{i,j}) \in $ that are independently {\em coherent} for each $r$, such that 
    	$$\sum_{r \leq r'} \sum_{(i,\Yboth_{v',j}) \in P_r} \LIS(X_{l(v')},\Yleft_{v',j}) + \LIS(X_{r(v')},\Yright_{v',j}) \geq \LIS(X_v,U_v) - 2.2\lambda |y \cap Y|$$
\end{claim}
%\ns{Change the claim to something like ``only 2 candidate $Y$-intervals are missing'' for $U$...}
\begin{proof}

    Define the following sets $P_r$:
    $$P_r \triangleq \left\{ (i,L_{i,j}^r \cup R_{i,j}^r) \mid L_{i,j}^r \cup R_{i,j}^r \subseteq U_i^r \wedge U_{2i-1}^{r/2} \setminus L_{i,j}^r < L_{i,j}^r \wedge U_{2i}^{r/2} \setminus R_{i,j}^r > R_{i,j}^r  \right\}$$
    
    Not that $P_r$ may not be {\em coherent} since it may have duplicate first coordinates. We fix that by removing duplicated $i$ arbitrarily (say, pick the smallest one).
    
    \ns{finish this...}
    
	We prove by induction on $r$. When $r=1$, we have at most 1 candidate interval $Y^1_{i,j}$ and hence $Y_i^1 = \emptyset \vee Y_{i,j}^1$ and the claim is immediate. Otherwise,
\end{proof}

==> dynamic-new.tex <==
\section{Fast data-structure for disjoint $\LIS$ extraction}\label{sec:dynamic}

In this section we show how to quickly break down a sequence into multiple disjoint $\LIS$ in an approximate greedy fashion, proving Thm~\ref{thm::dynamic_main}:


\begin{theorem}[Theorem~\ref{thm::dynamic_main}, restated]\label{thm::dynamic_main_res}
    There exists a data-structure that given a sequence of intervals $y \in \IC^n$, extracts a sequence of length $\Omega(\tfrac{|\OPT|}{\log n})$ in time $\tO(|\OPT|)$. The pre-processing time is $\tO(n)$
\end{theorem}


We use the following dynamic data-structure:\snote{Use Gawrychowski dynamic LIS - ensure their solution works for LIS over intervals, or see how to adapt it.}%\snote{Do we need to modify it for \reslis?}

\begin{theorem}\cite{?}\label{thm:disjoint_LIS_new}
	Given an input $\N^n$,
	%$\cE^n$, 
	there exists a {\em dynamic} data-structure with update time $(log(n) / \eps)^{O(1)}$, and with query time $O(|\OPT|)$, and which approximates the longest increasing sub-sequence up to $(1+\eps)$-factor
\end{theorem}

This does not suffice for our construction, since we need to perform $\LIS$ over $\IC$, which admit partial order relation only (as opposed to $\N$, which admits a total order relation). Hence, we build another layer on top of it.

\begin{lemma}\label{lm::dynamic_intervals}
    Suppose there exists a dynamic data-structure $\cD$ that supports updates in time $t_U$, and $\alpha$-approximate $\LIS$-queries in time $t_Q$ for $\LIS$ over the standard $\N^n$ domain. Then, there exists a data-structure $\cD'$ that given a sequence of intervals $y \in \IC^n$,  answers $O(\alpha \log n)$-approximate $\LIS$-extraction queries in time $\tO(t_Q + |\OPT| \cdot t_U)$. The pre-processing time is $n \cdot t_U + O(n \log n)$
\end{lemma}

We note that Theorem~\ref{thm:disjoint_LIS_new} and Lemma~\ref{lm::dynamic_intervals} immediately imply Theorem~\ref{thm::dynamic_main_res}

To prove Lemma~\ref{lm::dynamic_intervals}, we show first the following claim. 
\begin{claim}\label{corr::disjoint_LIS_elements}
	Suppose there exists a data-structure $\cD$ as above. Then, given an input $y \in \IC^n$, where all intervals $y_i$ are of measure $\mu(y_i) \in l[0.5,1]$ for some fixed $l$,
	%$\cE^n$, 
    one can construct a data-structure $\cD'(l)$ that  answers $2\alpha$-approximate $\LIS$-extraction queries in time $\tO(t_Q + \LIS \cdot t_U)$. The pre-processing time is $n \cdot t_U$.
\end{claim}

\begin{proof}
    Define the transformation $\varphi: \IC \rightarrow \N$ such that $\varphi(I) \triangleq \lfloor \min(I) / l \rfloor$. To pre-process $y$, compute $y' \triangleq \varphi(y)$, then insert all $n$ elements to $\cD$. Finally, we answer the extraction queries by $\LIS$-querying $\cD$, and outputting the longest common subsequence of $y$, restricted to the coordinates outputted by $\cD$, and removing each such element from the data-structure.
\end{proof}

Finally we prove Lemma~\ref{lm::dynamic_intervals}

\begin{proof}[proof of Lemma~\ref{lm::dynamic_intervals}]
Given an input $y \in \IC^n$ of arbitrary elements, we consider all 2n interval ``borders'', i.e., $E \triangleq \{\min(y_i),\max(y_i)\}_i$, and assume  $E$ is sorted (in time $O(n \log n)$). Next, we reassign each entry in $E$ according to its rank, and allowing double counting for same elements, i.e., $E={1,1,10,10,100}$ will be mapped to $f(E)={1,1,2,2,3}$. Next, we exponentially discretize the set of $n$ intervals by their length, such that $y(l) \triangleq \{y_i \mid \max(y_i)-\min(y_i) \in (0.5,1] l\}$, for $l \in \{2, 4, 8, \ldots, 2n \}$. Finally, we pre-process a data-structure $\cD(l)$ according to Claim~\ref{corr::disjoint_LIS_elements} for each $y(l)$. For $\LIS$-extraction, we query all $\cD(l)$ and extract the longest one, which costs another $\log(n)$-factor of approximation.
\end{proof}

==> dynamic.tex <==
\section{Data-structure for finding disjoint $\LIS$}

To find multiple disjoint $\LIS$-approx, we build a dynamic data-structure as follows:\snote{Use Gawrychowski dynamic LIS - ensure their solution works for LIS over intervals, or see how to adapt it.}%\snote{Do we need to modify it for \reslis?}

\begin{theorem} \label{thm:disjoint_LIS}
	Given an input $\cE^n$, there exists a {\em dynamic} data-structure that supports the following queries/operations:\snote{Ensure consistency between query time and runtime.}
	\begin{enumerate}
		\item Query $\textsc{ApproxLISMax}(M,l)$: Given a maximal value $M \in \N$, and sequence length $l$, output a value $m \in \N$ such that (i) $\LIS(y,X,[m,M]) \geq l$	; and (ii) $\LIS(y,X,[m',M]) < \lfloor(1+\epsilon) l\rfloor l$\snote{There are $2$ $l$'s here.} for all $m' > m$. The query time is $\poly(\tfrac{\log n}{\eps})$.
		\item Query $\textsc{ApproxLISMin}(m,l)$: Given a minimal value $m \in \N$, and sequence length $l$, output a value $M \in \N$ such that (i) $\LIS(y,X,[m,M]) \geq l$	; and (ii) $\LIS(y,X,[m,M']) < \lfloor(1+\epsilon) l\rfloor$ for all $M' < M$. The query time is $\poly(\tfrac{\log n}{\eps})$.
		\item $\textsc{GetMinRangeSeq}(M,l)$: Similar to $\textsc{ApproxLISMax}$, but also retrieves the actual sequence. The run-time is $O(l) + \poly(\tfrac{\log n}{\eps})$.
		\item $\textsc{RemoveElement}(i)$: given coordinate $i$, remove $(i,y_i)$ from the sequence. The run-time is $\poly(\tfrac{\log n}{\eps})$.
	\end{enumerate}
	The data-structure requires $n \cdot \poly(\tfrac{\log n}{\eps})$ space and preprocessing time. 
\end{theorem}

\subsection{Construction}
Given string $y$, we construct a binary tree where each character is a leaf and each node contains a sorted list of the elements \nnote{for intervals we need to sort twice, by min and by max}.

In addition, we store in each node and each length $l \in E_{1+\eps}(n)$ some increasing sequences $s_l$ of length $l$. We denote the set of such sequences as $\cS_{v,l}$. The sequences are stored with 2 identifiable parameters $m_L$ and $M_L$\snote{What does $L$ refer to? $l$ instead of $L$?} which are the min and max of the sequence set. The sequences are ``tight'', in the sense that all $I \subset [m,M]$\snote{Is this supposed to be a proper subset, to be consistent with \Cref{thm:disjoint_LIS}?} contain maximal lis $< l(1+\eps)$ (in particular, for $l < 1/\epsilon$, there is no sequence of length $l$ in any subinterval). 
The sequences are not stored directly on the node. Instead, it stored as pointers to (at most) 2 coherent sequences, which are $s_L \in \cS_{l(v),l_L}$
and $s_R \in \cS_{r(v),l_R}$ such that $l_L + l_R \approx l$. In addition to those pointers, we also store for each $s \in \cS_{v,l}$ ``meta-data'' $m^*,M^*$ which is the range of value for those sequences. The sequences in $\cS_{v,l}$ are slightly overlapping, such that every element can appear in $\poly(\log n/\eps)$ sequences for each $l$. 

\paragraph{Operations on nodes:}

First, we note that we allow the Theorem operations on any node in the tree representing a sub-string, and answer the theorem queries by querying the root. At each tree level we incur another $1+O(\eps)$ factor approximation, so the final approx is $(1+O(\eps))^{\log n}$. By setting $\eps' = \eps/\log(n)$, we fix the approximation as needed. We now describe more specific operations for each node.

\vspace{3mm}

\paragraph{Pre-processing procedure.} We initially build the sets $\cS_{v,l}$ as follows:

$\textsc{PreProcessNode}(v,l)$
This procedure updates the node sequences given (at most) 2 processed children. The runtime is $\tO(|v|)$.

We use the following subroutine:

$\textsc{IdentifyRangeTop}(v,l,T)$, $\textsc{IdentifyRangeBottom}(v,l,B)$.

These procedures are similar to $\textsc{ApproxLISMax}$,$\textsc{ApproxLISMin}$; with 2 differences: First, we {\em do not} assume the node is processed, only its children. Second, it outputs both a minimal and a maximal value $(m,M)$  %Given node $v$, a maximal value $M \in \N$, sequence length $l$, returns  output a value $m \in \N$ 
such that (i) $m \leq M \leq T$ (ii) $\LIS(y,X,[m,T]) \leq (1+\eps)l$; (iii) $\LIS(y,X,[m',M']) < \lfloor(1+\epsilon) l\rfloor$ for all $[m',M'] \subset [m,M]$. The query time is $\poly(\tfrac{\log n}{\eps})$.


\paragraph{Algorithm for $\textsc{IdentifyRangeTop}(v,l,T)$.}
For $l_R \in [\epsilon l, l] \cap \lfloor E_{1+\epsilon}(l)\rfloor$,\snote{Don't know what floor of a set means} let $l_L = l - l_R$, rounded up to the next power of $1+\epsilon$.
For each $l_R, l_L$ as above, compute $m_R(l_R) \gets \textsc{ApproxLISMax}(r(v),T,l_R)$, and then $m(l_L) \gets \textsc{ApproxLISMax}(l(v),m_R-1,l_L)$. 
We take the maximum $m^*$ of all $m(L_l)$ (if none exist, we output $\bot$).
We then do the same backwards using $m^*$ and \textsc{ApproxLISMin}, getting $M(r_R)$ for all $l_L,l_R$. we take the minimum of them $M^*$.
Finally, we output $(m^*,M^*)$.
We build a similar (backwards) algorithm $\textsc{IdentifyRangeBottom}(v,l,B)$

\paragraph{Algorithm for $\textsc{PreProcessNode}(v)$.}
For each $l \in \lfloor E_{1+\epsilon}(n)\rfloor$, we build the set $\cS_{v,l}$ as follows:
We iterate on maximal values in $v$. Initially, we set $M_v \triangleq \max{y_v}$. We Call $(m^*,M^*) \gets \textsc{IdentifyRangeTop}(v,l,M_v)$, and $(\cdot,M^-) \gets \textsc{IdentifyRangeBottom}(v,\lfloor l(1-\eps) \rfloor,m^*)$. We add the range $[m^*.M^*]$ to $\cS_{v,l}$, pointing to the corresponding sequences in the children, and set $M_v \gets M^-$ and iterate. We stop when $\textsc{IdentifyRangeTop}(v,l,M_v)$ outputs $\bot$.

%We with value rank a multiple of $\epsilon l$ (ie, $i \in Q_{\eps l/|v|}$ where is $Q$ is for quantile), and 

%build initially For each element $i \in v$ with value rank a multiple of $\epsilon l$ (ie, $i \in Q_{\eps l/|v|}$ where is $Q$ is for quantile), and each $l_R, l_L$ as above, compute $m_R(l_R) \gets \textsc{ApproxLISMax}(r(v),i,l_R)$\nnote{adapt to interval elements}, and then $m(l_R) \gets \textsc{ApproxLISMax}(l(v),m_R-1,l_L)$. Store the smallest interval $[m(l_R),i]$ in $v$ as a sequence of length $l$ with pointers to the corresponding sequences of length $l_R,l_L$.

\vspace{3mm}
$\textsc{RemoveElement}(v,i)$:
For $i \in v$, this procedure assumes the child of $v$ where $i$ belongs to was already processed $\textsc{RemoveElement}(i)$, and updates the node sequences at the current level. The run-time is $\poly(\log(n),1/\epsilon)$. We removing element, we call $\textsc{RemoveElement}(i,i)$ (ie, just on the leaf), and the procedure propogates up the tree)

\paragraph{Algorithm for $\textsc{RemoveElement}(v,i)$.} For each $l \in \lfloor E_{1+\epsilon}(n)\rfloor$ and $\cS_{v,l}$ where $i \in [m^*,M^*]$, we rebuild $[m^*,M^*]$ as we did in the pre-processing stage (note that by construction, there are at most $\poly(\log(n),1/\eps)$ such ranges for any single $i$, we then call $\textsc{RemoveElement}(\parent(v),i)$\nnote{check if need to remove redundant ranges to avoid over-overlapping...}.

\vspace{3mm}
\paragraph{Algorithms for $\textsc{ApproxLISMax}(v,M,l)$ and $\textsc{ApproxLISMin}(v,m,l)$.}
Simply return the range for sequence $s \in \cS_{v,l}$ which is closest to (but smaller/larger than) $M$.

\vspace{3mm}
\paragraph{Algorithm for $\textsc{GetMinRangeSeq}(M,l)$.} Recursively get the sequence elements using the pointers in $s \in \cS_{v,l}$ which is closest to (but smaller than) $M$.

%For $l_R \in [\epsilon l, l] \cap E_{1+\epsilon}(l)$, let $l_L = l - l_R$, rounded up to the next power of $1+\epsilon$.




==> genlis-ext.tex <==
\section{\genlis and \reslis Extensions Reductions, Proof of \Cref{lm::genlis_int_reduction,lm::reslis_int_reduction}}\label{sec:genlis_ext}


In this section we prove the \genlis and \reslis extensions reductions, namely  \Cref{lm::genlis_int_reduction,lm::reslis_int_reduction}.

\subsection{\genlis extension reduction}

%In particular, 
For the \genlis problem, we need to show two extensions:

\paragraph{\genlis over interval space.} Here we need to overcome the obstacle that the space $\IC$ admits a partial order relation only, as opposed to $\N$, which admits a total order relation. Our solution involves a mapping $\varphi: \IC \rightarrow \N$ that approximately preserves the overall $\LIS$ over all subsequences (with probability 1), and therefore also preserves the overall $\LIS$ over the genuine elements. We first note that such a mapping is applied a priori on the first coordinates of the input, and is not affected by the genuineness flags, nor does it require access to any genuineness samples. While we are unable to exhibit %do not manage to show
a single mapping for the entire space, we %are able to
show that one can reconfigure and decompose an arbitrary \genlis instance over intervals into $\log (k/\lambda)$ ``nicer'' instances $G_1,\ldots,G_{\log (k/\lambda)}$, which are mutually disjoint and whose union %altogether
covers most of the original $\genlis$ intervals (the unused intervals will be discarded at an ``additive error'' cost). Each such ``nicer instance'' is then be mapped to a \genlis instance over integers with a constant distortion over all its subsequences. We will use the following claim:

\begin{claim}\label{cl::intervals_similar}
	Define $\cI_\ell$ to be all intervals in $\cI$ of length %measure\snote{Replace with "length"? Let's not use technical terms if we don't need to?}\nnote{sure}
	$\ell\cdot[1,2)$ for some fixed $\ell \in \N$.
	Then, there exists a mapping $\varphi: \cI_\ell \rightarrow \N$, which can be computed in constant time, %$O(1)$-time,
	%$\cE^n$, 
   % For any $y \in \cI_\ell^n$, one can construct a data-dependent mapping $\varphi: \cI_\ell^n \rightarrow \N^n$, such that for any set of coordinates $U \subseteq [n]$:
   such that:
    \begin{enumerate}
    	\item For $I,J \in \cI_\ell$: $I < J \Rightarrow \varphi(I)<\varphi(J)$; and,
    	%	\item If $y \in \cI^m$ is an increasing sequence, then $\varphi(y)$ has an increasing subsequence of length $m/2$.
    	\item For all increasing sequences $y \in \N^m$ and all $q \in \cI^m$ s.t. $\varphi(q)=y$, $q$ must have an increasing subsequence of length $m/3$.%\blue{at least}
    	%\snote{Added "at least"} 
    	%\nnote{removed. I think adding at least just add confusion? if there is a sequence of length > $m/3$ must be also of precisely that}
   \end{enumerate}
 %   The mapping run-time is $O(1)$.%$O(n \log n)$.
\end{claim}

\begin{proof}
    We use the mapping $\varphi(I) \triangleq \lfloor \min(I)/\ell \rfloor$.\snote{added the argument of $\varphi$.} Then on one hand $I<J \Rightarrow \min(I)\leq \max(I) - \ell + 1 \leq \min(J) - \ell$ which implies $\varphi(I)<\varphi(J)$. 
    
   For (2), fix $y$ as above, and let $y^0,y^1,y^2$ be the sequence $y$ from integer elements satisfying, respectively, $(\mod 3) = 0, (\mod 3) = 1, (\mod 3) = 2$.\snote{I don't understand why there is no argument of the $\mod$ function. Is it the index of the sequence element or its value?}\ns{values} Let $q^0,q^1,q^2$ be the corresponding intervals of $q$. Then each such subsequence $q^i$ is clearly increasing, and since $|q^0| + |q^1| + |q^2| = m$, then at least one of them satisfies the length promise as well. 
\end{proof}

The final output will be the maximum \genlis over all integral instances: $\{\varphi_i(G_{i,1}),G_{i,2}\}_i$. This will cost us another $\log (k/\lambda)$-factor distortion.

% such that $\varphi(I) \triangleq \lfloor \min(I) / \ell \rfloor$. To pre-process $y$, compute $y' \triangleq \varphi(y)$, then insert all $n$ elements to $\cD$. Finally, we answer the extraction queries by $\LIS$-querying $\cD$, and outputting the longest common subsequence of $y$, restricted to the coordinates outputted by $\cD$, and removing each such element from the data-structure.

\paragraph{Empty Blocks.}
In some cases, we need to have an improved bound %where
for the case when the instance $g$ consists of 
at most 
$\eta n$ non-empty blocks (i.e., with more than 0 elements), each containing at most $k$ %$\leq k$ 
elements.
To obtain the improved bound, we implement a simulated algorithm $\genlis(g',\lambda')$, where $g'$ is defined as the input $g$ restricted to the non-empty blocks. We set parameters $n' \triangleq \eta n$ and $\lambda' \triangleq \lambda / \eta$, and while $T_{1/c_s(\lambda)}(g)$ allows us to access $O(\zeta / \lambda)$ random blocks of $g$, we note one can simulate $O(\zeta / \lambda')$ random blocks of $g'$ by {\em rejection sampling}. %The proof of correctness of this simulation is essentially identical to the proof for the usual case given below.

\newcommand{\rank}[0]{{\text{rank}}}

\begin{figure}[t]
    \setstretch{1.2}
  \begin{algorithm}[H]
    \caption{\genlis reduction}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{$g \in (\cI \times \zo)^{n \times k},\lambda\in [1/n,1]$, algorithm $\cA$ for \genlis over integers.}
		\KwOut{A number $\widehat{G} \in \left[0,n\right]$.
		}
		Let $y \gets g_1$ be the first coordinates of $g$. \\ %restricted to the non-empty blocks. \\
		
		Compute the set of integers $B \gets \cup_{i,j} \{\min(y_{i,j}),\max(y_{i,j})\}$.\\% be a set of integers.\\%\snote{I don't understand... Does this mean that "$B$ is a subset of integers defined as ... "?}\nnote{yes all the interval borders}
		
		Compute $a \in \cI^{n \times k}$ such that $a_{i,j} \gets [\rank_B(\min(y_{i,j})),\rank_B(\max(y_{i,j}))]$ for all $i,j$.\\
		
		\For{$(\ell,i) \in E_2(2k/\lambda) \times [n]$}
		{
			Compute $U_\ell \gets \{(i,j) \mid \mu(a_{i,j})\snote{Use either $\mu$ or $|.|$ consistently} \in [1,2) \cdot \ell\}$. \\
			Compute $b^{(\ell)} \gets \varphi_\ell(a(U_\ell)) \oplus g(U_\ell)_2$,\footnote{$\oplus$ is for direct sum} where $\varphi_\ell$ is the transformation of Claim~\ref{cl::intervals_similar}. 
		}
		\Return $\max_\ell \cA(b^{(\ell)})/3$.
		
\end{algorithm}
\caption{Description of the reduction algorithm.}
\label{fig:ALG_genlis_intervals}
\end{figure}


\begin{proof}[Proof of Lemma~\ref{lm::genlis_int_reduction}]
    Let $\cA$ be such that $\cA(b^{(\ell)})$ is a $(\alpha, \lambda n/2)$-approximation for $\genlis(b^{(\ell)})$ in time $t$. We need to show the reduction algorithm provides a $(O(\log (1/\lambda) \alpha),\lambda n)$-approx for $g$.
    
    Consider first intervals of measure $> 2k/\lambda$, which do not participate in any $b^{(\ell)}$. Any increasing subsequence of intervals contained in $[1,2nk]$ can have at most $\lambda n / 2$ intervals of such magnitude, hence by ignoring such intervals we ``lose'' at most  $\lambda n / 2$ additive error. Now, consider all low measure intervals $\leq 2k/\lambda$. Each such interval will participate in some $b^{(\ell)}$ and from Claim~\ref{cl::intervals_similar}, item 1, such interval will be mapped to an integer preserving its strict relation with all other intervals. Therefore, the lower bound holds for at least one $b^{(\ell)}$.
    
    For the upper bound, we use Claim~\ref{cl::intervals_similar}, item 2, to show that we always output an upper bound of the original interval sequence.
\end{proof}

\subsection{\reslis extension reduction}

For the \reslis problem, all we need to show is that one can ``ignore'' not too many exceptionally large blocks. The algorithm is the natural one:
\begin{enumerate}
	\item Using \Cref{cr::sampling_ds} and $T$, % and \blue{Fast Data Structure}\nnote{add such DS}, simulate sampling of $s \zeta$ uniformly random 
    sub-sample blocks $S \subseteq X$, each block independently with %iid
    %iid
    probability $\tfrac{\zeta}{\lambda |X|}$, and let %$W \gets $ set of values in  %$ and compute a set of coordinates 
    $W \gets \{(i,j) \in S \times [k] \mid y_{i,j} \in Y\}$.
	\item Compute $\Upsilon \gets$ the $0.6\lambda$ top-quantile of $\{|\{(i,j) \in W\}|\}_{i \in S}$.
    \item Run $\cA$. Whenever $\cA$ tries to access a block $i$ using $T$ we check first if $|y_{i,*} \cap Y| > \Upsilon$, and if so, we treat  the block as ``empty'' (say, by override).
   	\end{enumerate}

\begin{proof}[Proof of \Cref{lm::reslis_int_reduction}]
	\ns{proof tbw.}
\end{proof}


==> genlis_new.tex <==
%\input{genlis}
\subsection{\genlis - adaptation}

\ns{Add integrate this to above}

We now present our algorithm for $\genlis$.\snote{Put alg in a figure.}

\paragraph{Algorithm: $\genlis(g,\lambda,\gamma,T)$}

\begin{enumerate}
    \item Greedily and iteratively look for the maximal {\em pseudo-solutions}\snote{I don't think we've stated anywhere how to do this exactly, and what changes there are w.r.t \cite{rubinstein2019approximation}. Is that right?} each containing at least $\lambda n$ characters, %letters,
    generating solutions $P_1,\ldots,P_t$ for some $t \leq k/\lambda$.
    \item For $\ell \in 2^{[\log_2 k/\lambda]}$:
    \begin{enumerate}
    %\item let for $\ell \in 2^{[\log_2 1/\lambda]}$,
    \item let $\cP_\ell $ be the set of solutions of length $(l/2,l] \cdot \lambda n$, and let $U_\ell \triangleq \cup_{P \in \cP_\ell } P$.
    \item For $\zeta = O(\log n)$ and $\gamma = \lambda^{\delta}$ ($\delta$ is as previously defined), sub-sample $\max\{\gamma/k,1\} \zeta l$ %\nnote{can sample less for large $l$ if needed} \snote{I think we should sample $\gamma \zeta$ elements and multiply the first term in the max by $\ell$. Don't think we can afford $1/\lambda$ samples when $\ell \approx 1/\lambda$. I'm writing the correctness assuming this change.}
    single elements from %the union $P = \cup_i P_i$ 
    $U_\ell $ using $T$ and check if each one is genuine or not. Let $\kappa_\ell $ be the number of Genuine letters.\label{alg_gen_lis_sampling}
    \end{enumerate}
    \item Compute and output:%\snote{Should the first term be $|P|\kappa / (\gamma \zeta)$? I don't think the current expression is unbiased; it seems to be an overestimation by a factor of $n/|P|$ (assuming the Gen-LIS is a subset of $P$, which we have to prove.)}
    %\nnote{You right. The $n$ is there from before when originally we wanted lower bound of OPT. Now we care to upper bound, hence $|P|$ should be used indeed. and proof for all genlis elements minus additive error is easy/trivial since if the longest remaining LIS (not necessarily genuine) is $L$, then we know we are missing at most $L$ elements in the optimal genlis as well...} %\snote{Don't understand what the third argument $(\lambda \gamma)$ in the $\reslis$ is supposed to be. Doesn't $\reslis$ take only 2 arguments - the sequence ($y(P)$ in this case) and the range $(\N \times \{1\}$)?}\nnote{no, it also takes the additive error parameter $\lambda$, see the list of inputs in the algorithm for $\reslis$ in next subsection}
    $$\max_\ell \max\left\{\tfrac{\lambda n \kappa_\ell }{\gamma \zeta},\reslis\left(y(U_\ell ),\N \times \{1\},\lambda,T \right)\right\}.$$ 
\end{enumerate}

==> improved_approx.tex <==
\section{Improved approximation - $\genlis$ reduction}
 
\subsection{Setup and Definitions}
 
Define the $\reslis_{n,m}$ as before, ie $\LIS_Y(y)$ for input $y \in \N^n$ and range $Y$. Here we define $m \triangleq |y \cap Y|$.

Define the $\genlis_n$ problem as follows: 
The input is a number string where each number receives an additional flag whether it is genuine or not, ie  $y \in (\N \times \{\uncor,\cor\})^n$ \nnote{we may need to have the first coordinate as $I^n$ for interval space $I$}. One receives unrestricted access to the string (ie, the first coordinates) but must ``pay'' to check wether a number is genuine or not. The goal is to estimate $\LIS_{\N \times \{1\}}(y)$ (alternatively, $\LIS(y_1 \odot y_2)$).\nnote{$\odot$ denotes the Hadamard coordinate-wise Multiplication}

One can observe that $\genlis_n \subseteq \LIS_n \subseteq \reslis_n$.%\snote{Confused about the second inclusion; I don't understand how restricting the set of $y$-values can increase the LIS. Also, this subset notation doesn't sync up with the rest of the paper; $\LIS(y)$ already represents the length of the LIS in $y$, and not the longest increasing sequence itself.}




\subsection{Main Theorems}

\begin{theorem}[$\genlis$ recursive hypothesis]\label{thm::gl_rec}
	Fix $\lambda, n$. Suppose, for some fixed functions $a_s, c_s$ on $\R \rightarrow \R$, there exist a randomized algorithm $\cA_{SL}$ that $(a_s(\lambda_s),\lambda_s m_s)$-approximates $\reslis_{n_s,m_s}$ using $c_s(\lambda_s) \cdot \tfrac{n_s}{\lambda_s m_s}$ complexity 
	 for all $n_s < n$ and 
	 $\lambda_s \geq \lambda$. 
	 Then, for any $\gamma\ge1$, one can produce a $(a_s(\gamma \lambda) + \gamma, \lambda n)$-approximation for $\genlis_n$ using $\tilde{O}(\gamma) + c_s(\gamma \lambda)\cdot \gamma$ genuine tests.%\snote{Not clear to me how we are obtaining a bound on the "number of genuine tests" from the sample complexity of \reslis (which is for a traditional LIS problem).}\nnote{because a genuine test represent a recursive test over a candidate interval and we bound those.}
	 Moreover, the algorithm has run-time $O^*(n)$.\snote{I think any LIS algorithm's run-time should be trivially bounded by $\tilde{O}(n)$; why do we need $O^*(n)$? What am I missing here?}\nnote{for time complexity we want to have $O^*(n)$ and not some of the hypothesis testing algorithms from above...}
\end{theorem}


\begin{theorem}[$\reslis$ recursive hypothesis]\label{thm::sl_rec}
	\snote{It seems like $\lambda_g, \lambda_s$ depend on $\lambda$, but then later $\lambda$ is set to $\lambda_g \lambda_s$ - circular. EDIT: I understand it's not actually circular, but the description implies that definition is circular. Will rewrite.} Fix $\lambda, n$. Suppose, for some fixed functions $a_g, c_g$ and $a_s, c_s$ on $\R \rightarrow \R$, there exists algorithms $\cA_{GL}$ that $(a_g(\lambda_g),\lambda_g n_g)$-approximates $\genlis_{n_g}$ using $c_g(\lambda_g)$ complexity,
	 and $A_{SL}$ that $(a_s(\lambda_s),\lambda_s m_s)$-approximates $\reslis_{n_s,m_s}$ using $c_s(\lambda_s)\cdot \tfrac{n_s}{\lambda_s m_s}$ complexity 
	 for all $n_g,n_s \leq n^{1-\delta}$ (for some constant $\delta$\nnote{tbd}) and 
	 $\lambda_g,\lambda_s \geq \lambda$. 
	 Then we can produce a $(\alpha, \lambda m)$-approximation for $\reslis_{n,m}$, where %$n= n_g n_s$, 
	$\alpha = \polylog (1/\lambda) \cdot a_g(\lambda_g) a_s(\lambda_s)$ for some $\lambda=\lambda_g \lambda_s$ using $\polylog (n) \cdot c_g(\lambda_g) \cdot c_s(\lambda_s) \cdot \tfrac{n}{\lambda m}$ queries.
\end{theorem}
\begin{proof}
    $\lambda_g$ is the fraction of candidate intervals participating in the total $\LIS$. $\lambda_s$ is the local $\lambda$ within the candidate intervals we need once we recurse %recourse
    on a candidate interval. Overall, we reduce the problem to find $\lambda_g$ LIS of candidate intervals, each having $\lambda_s$-local LIS, where $\lambda_g \lambda_s \approx \lambda$.
    
\end{proof}


\ns{add the probability of success to the above theorems...}


\begin{corollary}
	Fix $n$. For any $\lambda$, there exists a randomized algorithm $A_{SL}$ that $(\tO(2^{\sqrt{\log (1/\lambda) \cdot \log\log (1/\lambda) / \epsilon}}),\lambda n)$-approximates $\reslis_n$ using $O^*(\lambda^{-2})$ queries.
\end{corollary}
\begin{proof}
\aanote{change t into k, and k into something else}
\paragraph{Correctness:}
	We prove by induction. For the base case where $\lambda=\Omega(1)$... \ns{add base case.}
	
	Otherwise, for $k=1/\lambda$, we get by induction approximation $a(k) = \polylog(k) \cdot \max_{t} (a(k/t) \cdot \gamma \max\{a(t/\gamma) ,\gamma\})$, and complexity $c(k) = \polylog(n) \cdot \max_{t} (c(k/t) \cdot \max\{\gamma \cdot c(t/\gamma),t\})$ for our choice of $\gamma$.
	
	Another way to define the recursion relation is as follows:
	
	$$a(n,b,k) = \polylog(k) \cdot \max_{t} (a(n/b,b,k/t) \cdot \max\{a(b,b^\eps,t/\gamma),\gamma\}$$
	
	for any $k,n,b$:
	$$a(1,1,k) = O(1)$$
	
	$$a(n,b,1) = O(1)$$
	
	For $b \geq n^\epsilon$, we can fix $\gamma = t^\delta$, and this resolves to:
	
	$$a(n,b,k) = \log(k)^{O(1/\epsilon)}\prod_{t_1,\ldots,t_{1/\epsilon}: t_1 \cdot t_2 \cdot \ldots \cdot t_{1/\epsilon} = k} \max\{t^\delta,a(b,b^\epsilon,t^{1-\delta})\}$$
	
	We now assume by induction that $a(m,m^\eps,t) \leq \log^{O(1/\epsilon)}(t) t^\delta$ for any $t < k$. This further resolves to:
	
	$$a(n,b,k) = \log(k)^{O(1/\epsilon)}\prod_{t_1,\ldots,t_{1/\epsilon}: t_1 \cdot t_2 \cdot \ldots \cdot t_{1/\epsilon} = k} \max\{t^\delta,t^{(1-\delta)\delta} \log^{O(1/\epsilon)}(t)\} = \log(k)^{O(1/\epsilon)} \cdot k^\delta$$
	
	as long as $t^{(1-\delta)\delta} \cdot \log^{O(1/\epsilon)}(t) \leq t^\delta$.
	
	Hence we need $\delta^2 \geq \tfrac{\log(\log^{O(1/\epsilon)} t)}{\log t} = O(\tfrac{\log\log t}{\eps \log t})$.
	
	overall, we have $\tO(k^{\sqrt{\tfrac{\log\log k}{\eps \log k }}}) = 
	\tO(2^{\sqrt{\log k \cdot \log\log k / \epsilon}})$	approximation.

\paragraph{Complexity:}
\ns{work in progress....}
similarly, for complexity we have 
	$$c(n,m,b,k) = \polylog(n) \left( b +\max_{t} (c(n/q,m/b,k/t) \cdot t^\delta \cdot c(b,b^\eps,t^{1-\delta})\right)$$
	
	for $b=n^\eps k \cdot n/m$ and some $q > b t$.
	
	Also, for any $k,n,m,b$:
	$$c(1,1,k) = O(1)$$
	
	$$c(n,b,1) = \tO(1)$$
	
	Assume by induction for smaller $n,m,k$ we have the $O^*(k^2) \cdot n/m$ bound, then:
	
	$$c(n,m,b,k) \leq O^*(k) \left( 1 +k/t^2 nt/m) \cdot O^*(t^{2-\delta})\right) \leq \text{blabla...}$$
	
	\ns{here...}
%	
%	for any $k,n$:
%	$$a(1,k) = O(1)$$
%	
%	$$a(n,1) = O(1)$$
%	
%	where $n',n'' \leq n^{1-\delta}$ and $n' \cdot n'' \approx n$.
%	
%	Say we had $a(k) = C \cdot \max_t a(k/t) \cdot a(t)$
%	this is at least $a(k) = C \cdot a(\sqrt{k})^2 = C^{\log k} = k^{\log C} = \poly(k)$.
%	
%	So we need $\gamma$.
%	
%	For example, we can set $\gamma = \gamma(t) = t^\delta$ and obtain something like $\leq 2^{\log^{1-\delta}(k)} = k^{\delta} + k^{o(1)}$.
%	
%	


\ns{Alex says edit distance to $\ell1$ embedding has something similar, will yield $2^{\sqrt{\log 1/\lambda}}$ more or less...}


	\ns{$t$ would be $1/\lambda_g$ which is arbitrary. $a_s(\lambda_s) = a(k/t)$, $a_g(\lambda_g) = \min_\gamma(a(t/\gamma) + \gamma))$}
	
	
	\ns{add $n$ dependency on complexity. $\gamma$ needs to be the same for complexity and approximation. prove the recursion formula yields the bound and derive the exact formula for $\lambda^{-o(1)}$.}
\end{proof}

\input{genlis}

\vspace{3mm}

\subsection{Algorithm for $\reslis$, proof of Theorem~\ref{thm::sl_rec}}

Now we present our algorithm for the $\reslis$ problem. The algorithm works in a similar fashion to Section 7, with 2 important differences. First, to allow for smooth reduction to $\genlis$, we pair only one $j$ for each $r,i$; in particular, a pseudo-solution will consist of (at most) 1 candidate interval $Y_{i,j}$ for each block $X_i$.% (to allow that, we analyze over multiple radiuses $r$). %(note this makes the invariants Lemma slightly more subtle (part 4 in particular)). 
In order to force at most one candidate interval per block, we generate the $\genlis$ instance where each coordinate represent a $(X_i,Y_{i,j})$ pair: the $X_i$ are sorted in order, but the $Y_{i,j}$ are sorted in {\em descending order} (for a fixed $i$). This results ensures at most 1 element per $x$-block can participate in any $\genlis$ increasing subsequence. %(alternatively,  1 candidate interval per block can participate in a pseudo-solution). 
To allow that, we make a few adjustments to how we define $x$ and $y$-intervals. First, we define $X_i$ over multiple radiuses, denoted $X_i^r$. Second, candidate intervals is defined based on samples from a slightly larger radius. Last, we allow multiple samples in a candidate interval from such larger radius, as long as:
\begin{enumerate}
	\item There are no samples within the interval for the smaller radius (to ensure the instance is "sparse" enough).
	\item One of the following must hold: either a sample of the current radius is on (at least) one of the edges, or the number of samples is an exponent of 2. This guarantee ensures not too many candidate intervals.
\end{enumerate}

Overall, our algorithm proceeds as follows:

%We observe that \Cref{thm:main} follows from \Cref{thm:technical}. To see this, we call \ALG with input $X=[n],Y=\N$, the input sequence $y$, and $\lambda$, where $\LIS(X,Y)=\lambda n$, and then scale the output $\textsf{out}$ of \ALG suitably.

\begin{figure}[t] \label{fig::ALG_reslis}
\setstretch{1.2}
  \begin{algorithm}[H]
    \caption{\reslis}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{intervals $X, Y \subset \N$, a string $y \in \N^{|X|}$, block size $b$ %(assume for now an interval\ns{we expect most blocks LIS to intersect with ``one part'' of $Y$ and in any case should be easily reducible to that})
and parameter $\lambda \in (1/n,1)$.}
		\KwOut{A number $\widehat{L} \in \left[\LIS(X,Y) \cdot \lambda^{o(1) }- \lambda |y \cap Y|, \LIS(X,Y) \right]$.%\snote{Does this mean $1/\lambda^{o(1)}$?}\nnote{Yes!}
		}
		
		Set $b \gets n^\eps / \lambda$.\\ %\ns{I think $b = n^\eps$ suffices.} 
   % and $t \gets O_\epsilon(\polylog(1/\lambda)/\lambda)$.\\
    If $|X| < b \log n$, compute and return $\widehat{L}=\LIS(X,Y)$ exactly.\\
    Otherwise, sample $s= b \cdot \log n$ elements $(w_1, y_{w_1}), (w_2, y_{w_2}), \cdots, (w_s, y_{w_s})$  %$x$-coordinates 
    uniformly from $X \cap y^{-1}(Y)$ by {\em rejection sampling}, where $w_1 < w_2 < \cdots < w_s$.\\ 
        \For{$r \in 2^{[\log_2 1/\lambda]}$}{
     Let $X^r_1,\ldots,X^r_{b/r}$ be a partition of $X$ into $b/r$ consecutive disjoint intervals each consisting of $r\cdot \log n$ (non-rejected) samples, i.e., $X^r_i = [w_{(i-1)r\log n+1}, w_{ir\log n}]$.\footnote{Note that we do not impose that $X_i$'s have equal width.}  \\
     For $i \in [b/r]$, let $\cS^r_i=(y_{((i-1)r+j)\log n})_{j\in[r]}$ be the sequence of $y$-values of the $r$ samples in $X^r_i$ whose order is a multiple of $\log n$. \\
     %sorted in descending order; %We assume (by construction) such $\cS^r_i$ are in decreasing order;
     $\cY_i^r \gets \partition(r,i)$.\\%\textsc{PartitionY}(r,i)$. \\
     %$\{Y^r_{i,j}\}_{j\in [r-1]} \triangleq [\cS^r_i(j+1),\cS^r_i(j)]$ be the candidate intervals for block $i$ (again, in descending order).\nnote{we used decreased order to ``force'' the longest $\genlis$ having at most one $j$ for each $i$} \\
      \For{$k \in 2^{[\log_2 1/\lambda]}$}{
  %     Let $g \triangleq Y_{1,1},Y_{1,2},\ldots,Y_{1,r-1},Y_{2,1},\ldots,Y_{b/r,r-1}$ be a $\genlis_b$ input string.  \\
       Let $g_{r,k} \triangleq \left[\left(Y^r_{i,j}\nnote{this is abuse of notation since $\genlis$ is defined on numbers and not intervals. I will see if I can reduce to fixed numbers and if not, will define inputs for both $\genlis$ and $\reslis$ to be of interval spaces to avoid such an issue. in any case dont expect an issue here...},\1\left[\reslis\left(X^r_i,Y',\tfrac{1}{k}\right) > \tfrac{|y \cap Y|}{bk}\right]\right)\right]_{i \in [b/r],Y' \in \cY_i^r}$. \nnote{We first order by $i$ ascending, then by $\cY_i^r$ descending. Note that we use interval input rather than numbers for now. Formalize this better!}\\
  %     Let $\1[\reslis(X_i,Y_{i,j},1/k) > 1/k]$ be the genuine value of each element of $g$. \\
       Compute $L_{r,k} \gets \genlis(g_{r,k},k \lambda) \cdot 0.9 \tfrac{|y \cap Y|}{bk}$.\\}}
    Return $\widehat{L} \gets \max_{r,k} L_{r,k}$.%\cdot \log^2 1/\lambda$.
\end{algorithm}
\end{figure}

\begin{figure}[t] \label{fig::ALG_partY}
\setstretch{1.2}
  \begin{algorithm}[H]
    \caption{\partition}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{Integers $r \in 2^{[\log (1/\lambda)]}$ and $i \in [b/r]$.} %(assume for now an interval\ns{we expect most blocks LIS to intersect with ``one part'' of $Y$ and in any case should be easily reducible to that})
%and a sequence of $y$-values of length $S^r$.}
		\KwOut{An interval sequence $\cY$.}%\\
		Let $\cS = \cS^r_i$, and $\cS^p = \cS^{2r}_{\lceil i/2 \rceil}$.\\
     $\cY \gets \left\{[a,b] \in \cS^p \mid (a,b) \cap \cS = \emptyset \wedge \left([a,b] \cap \cS \neq \emptyset \vee |[a,b) \cap \cS^p| \text{ is power of 2.} \right)\right\}$ \\
	return $\cY$
\end{algorithm}
\end{figure}


\ns{The block size $b$ should be fixed when recursing in genuine tests, but should become smaller when converting the $\genlis$ to $\reslis$... need to write that down...}


\subsubsection{Analysis}

%We will analyze the lower bound and upper bound of our estimator.
Before analyzing the estimator $\widehat{L}$, we first prove some essentials invariants of our construction:

\begin{lemma}\label{lm::reslis_invariants}
    Fix $X,Y, y$ inputs. W.h.p, all the following invariants holds for $\reslis$ algorithm:
    \begin{enumerate}
    	\item For all $r,i$: $|y(X^r_i) \cap Y| \in [0.9,1.1]\tfrac{r|y \cap Y|}{b}$.
    	\item For all $r,i$ and all $Y' \in \cY_i^r$: $|y(X^r_i) \cap Y'| \leq 1.1 \tfrac{|y \cap Y|}{b}$. 
    	\item For all $r$ and all sets of pairs $\{(i,Y')\}_i$ that are {\em coherent}, we have $\sum_i \LIS(X_{i},Y \cap Y') \leq \LIS(X,Y)$.
		\item There exists interval sets $\widetilde{\cY^r_i} \subseteq \cY^r_i$ such that: (i) $|\widetilde{\cY^r_i}| \leq 3$; (ii) For all $r$: $\{(i,\cup_{Y \in \widetilde{\cY^r_i}} Y)\}_{i}$		is a coherent set; and (iii)
		%:i \text{ is even}}$ and $\{(i,\cup_{Y \in \widetilde{\cY^r_i}} Y)\}_{i:i \text{ is odd}}$ are
		% which are {\em coherent} for each $r$, such that %$(i,Y_{i,j}) \in $ that are independently {\em coherent} for each $r$, such that 
 %   	$$\sum_r \sum_{(i,L^r_{i,j} \cup R^r_{i,j}) \in P_r} \LIS(l(X^r_{i}),L^r_{i,j}) + \LIS(r(X^r_{i}),R^r_{i,j}) \geq \LIS(X,Y) - 2.2\lambda |Y \cap y|.$$
%    	\item There exists sets of pairs $\{(i_r,Y_{i,j(i_r)})\}_i$ that are independently {\em coherent} for each $r$, such that 
    	$$\sum_r \sum_i \sum_{Y' \in \widetilde{\cY^r_i}}\LIS(X^r_i,Y') \geq \LIS(X,Y) - 2.2\lambda |Y \cap y|.$$
    \end{enumerate}
\end{lemma}

We now analyze the correctness and complexity of our algorithm, proving Theorem~\ref{thm::sl_rec}:

\begin{proof}[Proof of Theorem~\ref{thm::sl_rec} using Lemma~\ref{lm::reslis_invariants}]

%	\ns{fix/polish using new defs / invariants...}
	
%	Let $l^r_{i,j} \triangleq \LIS(X^r_i,Y^r_{i,j})$. 
	For all $i$ and all $Y' \in \cY_i$, let $l^r_{i,Y'} \triangleq \LIS(X^r_i,Y')$. 
	By Lemma~\ref{lm::reslis_invariants} (4), we have for some $r^*$ a coherent set of pairs $P_{r^*} \subseteq \{(i,Y')\}_{i, Y' \in \cY_i}$ such that:
	$$\sum_{(i,Y') \in P_{r^*}} l^{r^*}_{i,Y'} \geq \tfrac{\LIS(X,Y) - 2.2 \lambda |Y \cap y|}{3\log 1/\lambda}$$
	
%	\ns{here...}
	
	Hence, fix $a_s > 1$.\snote{Very confusing notation. Is $a_s$ a number or a function? It's used for both purposes in this proof.} There must exists some $k^*$ for which:
	
	$$\sum_{(i,Y') \in P_{r^*}} \1[l^{r^*}_{i,Y'} \geq \tfrac{2a_s |y \cap Y|}{ bk^*}] \geq \tfrac{bk^*}{2a_s |Y \cap y|} \cdot \tfrac{\LIS(X,Y) - 2.2\lambda|Y \cap y|}{3\log^2 1/\lambda}$$
	
    Now, let us first argue correctness. Recall the following statement guarantees for each $(i,Y')$ pair:
    \begin{enumerate}
        \item Let $\widehat{l^{r^*}_{i,Y'}}$ be the output of $\reslis(X^{r^*}_i,Y',\tfrac{1}{k^*})$. Then $\widehat{l^{r^*}_{i,Y'}}$ is a $(a_s(\tfrac{1}{k^*}),\tfrac{|y \cap Y'|}{k^*})$-approximation for $l_{i,Y'}^{r^*}$.
        \item The output of $\genlis(g_{r,k},k \lambda)$ is a $(a_g(\lambda k^*),\lambda b k^*)$-approximation for $\sum_{(i,Y') \in P_{r^*}} \1[\widehat{l^{r^*}_{i,Y'}} \geq \tfrac{|y \cap Y|}{bk^*}]$.
    \end{enumerate}
     
     We use the above to derive the following lower bound on $ L_{r^*,k^*}$:
    
    \begin{align*}
        L_{r^*,k^*} &\geq \left(\tfrac{1}{a_g}\sum_{(i,j) \in P_{r^*}} \1\left[\widehat{l^{r^*}_{i,Y'}} \geq \tfrac{|y \cap Y|}{bk^*}\right] - \lambda b k^* \right) \cdot 0.9 \tfrac{|y \cap Y|}{bk^*} \\
        &\geq \sum_{(i,Y') \in P_{r^*}} \left(\tfrac{1}{a_g}\1\left[l^{r^*}_{i,Y'} \geq a_s\left(\tfrac{|y \cap Y|}{ bk^*} + \tfrac{|y \cap Y_{i,j}|}{k^*}\right)\right] - \lambda b k^* \right) \cdot 0.9 \tfrac{|y \cap Y|}{bk^*} \\
        &\geq \tfrac{1}{a_g} \sum_{(i,Y') \in P_{r^*}} \1\left[l^{r^*}_{i,Y'} \geq \tfrac{a_s \cdot|y \cap Y|}{ bk^*} + \tfrac{1.1 a_s |y \cap Y|}{b k^*}\right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9 \lambda |y \cap Y| \\
    &\geq \tfrac{1}{a_g}\sum_{(i,Y') \in P_{r^*}}\1\left[l^{r^*}_{i,Y'} \geq \tfrac{2.1a_s \cdot|y \cap Y|}{ bk^*} \right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
    &\geq \tfrac{1}{a_g} \cdot  \tfrac{bk^*}{2.1a_s |Y \cap y|} \cdot \tfrac{\LIS(X,Y) - \lambda|Y \cap y|}{\log^2 1/\lambda} \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
    &> \tfrac{1}{2.5 a_s a_g \log^2 1/\lambda} \cdot \LIS(X,Y) - \lambda |y \cap Y|
    \end{align*}
    
   % \ns{take care of the small extra additive factor (say, by adding another 2 factor in the denominator. Add complexity analysis. Add the extra constant to Theorem.}
    
    \ns{Think if can get this down to $1+\eps$...}
\end{proof}

%\subsubsection{Correctness Analysis}
%\subsubsection{Complexity Analysis}

\subsubsection{Proof of Lemma~\ref{lm::reslis_invariants}}
%\ns{@Sandip - can you please take care of that?}

%for 4: use 7.3 and show by induction on the radius, divide and conquer on both sides and the overlap interval using the larger radius

\snote{Items 1,2,3 in Section 9; import from there, edit notation.}\paragraph{Proof of item (4):}
For $t \in [n^\eps]$, Consider a binary tree $T_t$ of height $\log_2 1/\lambda$ where each node represent a $(r,i)$-pair as above. We use $X_v$ for interval $X_i^r$ and $\cY_{v,j}$ for candidate $y$-intervals. The leaves $v^1_i$ represent the smallest-size intervals $X_i^1$. For each node $v^r_i$ %represent interval $X^r_{i}$ with 
we connect with the children are $v^{r/2}_{2i-1}$ and $v^{r/2}_{2i}$ as children. Note that each $X_v$ node is a concatenation of $X_{l(v)}$ and $X_{r(v)}$. The roots are $v_t^{1/\lambda}$.



    To define the sets $\widetilde{\cY_i^r}$ we make the following definitions and notations:
    

    
    \begin{definition}
    	Fix a finite set of intervals $S \subseteq \cI$. 
    	The {\em top interval} $\top(S)$ is the interval which contains the maximal value in $\cup_{I \in S} I$ and is not contained in any other interval in $S$.
    	 Similarly, the {\em bottom interval} $\bot(S)$ is the interval which contains the minimal value in $\cup_{I \in S} I$ and is not contained in any other interval in $S$. 
    \end{definition}
    
   
   Next, for optimal increasing subsequence $y(X^*)$ for $\LIS(X,Y)$, let $M_i^r \triangleq \max\{y(X_i^r \cap X^*)\}$ be the maximal value of $y(X^*)$ in $X_i^r$ (by convention, $M^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_i^r \triangleq (M_{j}^r,M_i^r]$ for the largest $j<i$ such that $M_j$ is defined (similarly, let $U^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_v = U_i^r$ for $v=v_i^r$.
   
   We define the following candidate intervals:
   %containing all $\reslis$ values of $X_v$, ie:
%$$U_v \triangleq [\min y(X^* \cap X_v),\max y(X^* \cap X_v)]$$


    $$Y_v^\top \triangleq %\left\{ Y_{v,j} \mid 
    \top(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
    
    %} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} < Y_{v,j} \right\}$$

   % $$Y_v^\top \triangleq \left\{ Y_{v,j} \mid 
   % \top(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
   $$Y_v^\bot \triangleq %\left\{ Y_{v,j} \mid 
    \bot(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
    
    %\triangleq \left\{ Y_{v,j} \mid Y_{v,j} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} > Y_{v,j} \right\}$$

    $$Y_v^+ \triangleq %\left\{ Y_{v,j} \mid 
    \top\nnote{$\top$ can be $\bot$ as well, as they are equal for this set.}\left(\left\{Y \in \cY_v \mid Y \subseteq U_v \wedge U_{l(v)} \setminus Y <  Y \wedge U_{r(v)} \setminus Y > Y  \right\}\right)$$
 

Now for each $v=v_{r,i}$ in the tree, let $\widetilde{\cY_v}  = \widetilde{\cY_i^r} \triangleq \{Y_v^\top,Y_v^\bot,Y_v^+\}$. %\{ \top(\{Y \in \cY_v \mid Y \subseteq U_v\}), \bot(\{Y \in \cY_v \mid Y \subseteq U_v\})\}$ .%for even $i$ and $\cY_i^r \triangleq \{Y_v^c,Y_v^o\}$ for odd $i$.

To prove the Lemma, we claim the following:

\begin{claim}\label{cl::coherent_sets}
	For each $r$, the set $(i,\cup_{Y \in \widetilde{\cY_i^r}} Y)$ is coherent.
\end{claim}
\begin{claim}\label{cl::sum_of_descendants}
 For each $v$:	
		$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,\cup_{Y \in \cY_v: Y \subseteq U_v} Y)$$
\end{claim}

To complete the argument, % using Claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}
all that is left is to apply Claim~\ref{cl::sum_of_descendants} on the roots, and get the following bound:

\begin{align*}
\LIS(X,Y) &= \sum_i \LIS(X_i^{1/\lambda},U_i^{1/\lambda}) \\
 &\leq \sum_i \left(\LIS(X_i^{1/\lambda},\cup_{Y' \in \cY_i^{1/\lambda}: Y' \subseteq U_i^{1/\lambda}} Y') + |y(X_i) \cap U_i^{1/\lambda} \setminus \cup_{Y' \in \cY_i^{1/\lambda}: Y' \subseteq U_i^{1/\lambda}} Y'| \right) \\
 &\leq \sum_i \left(\sum_r \sum_{Y' \in \widetilde{\cY_i^r}}\LIS(X_i^r,Y') + 2.2\lambda  |y(X_i) \cap Y|\right)	\\
 &\leq \sum_i \sum_r \sum_{Y' \in \widetilde{\cY_i^r}}\LIS(X_i^r,Y') + 2.2\lambda  |y \cap Y|	
\end{align*}

as needed.

We now prove claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}.

\begin{proof}[Proof of Claim~\ref{cl::coherent_sets}]
	By definition, we have each $Y \in \widetilde{\cY_i^r}$ is contained in $U_i^r$, hence $\cup_{Y \in \widetilde{\cY_i^r}} Y \subseteq U_i^r$. Now, clearly, for any $r$, the set $\{(i,U_i^r)\}_i$ is coherent, and therefore the set $\{(i,\cup_{Y \in \widetilde{\cY_i^r}} Y )\}_i$  is coherent as well.
\end{proof}

The second claim requires more work.

\begin{proof}[Proof of Claim~\ref{cl::sum_of_descendants}]
	Let $Y_v^* \triangleq \cup_{Y \in \cY_v: Y \subseteq U_v} Y = [\min\{\cS^*_{\parent(v)}\},\max\{\cS^*_{\parent(v)}\}]$. We need to show:
	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,Y_v^*)$$
	
	 We prove by induction on the tree level. For leafs, $|\cY_v|=1$ and hence if such interval is contained in $U_v$, then $\widetilde{\cY_v} = \{Y_v^*\}$.
	
	For other nodes, let $\cS^*_v \triangleq \cS_v \cap U_v$ be the set of sampled coordinates in range. Now consider the following cases:
	
		\paragraph{There are samples in range:} If $\cS^*_v \neq \emptyset$, then $Y_v^\top = [\max\{\cS^*_v\},\max\{\cS^*_{\parent(v)}\}]$ and $Y_v^\bot = [\min\{\cS^*_{\parent(v)}\},\min\{\cS^*_v\}]$. This implies 
		$$\LIS(X_v,Y_v^*) \leq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) + \LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\}))$$
		
		The last quantity needs to be broken down further.
		Let $\cSleft_{v} = \cS_v \cap U_{l(v)}$ and $\cSright_{v} = \cS_v \cap U_{r(v)}$. Since $U_{l(v)}$ and $U_{r(v)}$ are consecutive, we have $\cSleft_v \cup \cSright_v = \cS^*_{v}$. %\ns{fix this later by defining the $U_v$ to have no gaps}, 
		Therefore $Y_v^+ = [\max\{\cSleft_v\},\min\{\cSright_v\}]$. Overall:
		
			\begin{align*}
			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			&\leq \LIS(X_v,Y_v^+) \\
			&+\LIS(X_{l(v)},(\min\{\cSleft_v\},\max\{\cSleft_v\}))  \\
			&+\LIS(X_{r(v)},(\min\{\cSright_v\},\max\{\cSright_{v}\}))				
			\end{align*}
			
			\ns{Check if need to change $\LIS(X_v,Y_v)$ to $|y(X_v \cap X^*)|$ throughout.}
			
			Note that by definition, $Y_{l(v)}^* = [\min\{\cSleft_v)\},\max\{\cSleft_v\}]$ and $Y_{r(v)}^* = [\min\{\cSright_v\},\max\{\cSright_{v}\}]$, hence we get:
		
	$$
			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			\leq \LIS(X_v,Y_v^+) 
			+\LIS(X_{l(v)},Y_{l(v)}^*)  
			+\LIS(X_{r(v)},Y_{r(v)}^*)				
$$

which by induction can be upper bounded by:
$$
\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			\leq \LIS(X_v,Y_v^+) 
			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)$$
			
Hence we conclude 

\begin{align*}
\LIS(X_v,Y_v^*) 
&\leq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) + \LIS(X_v,Y_v^+) 
			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)\\
		&= \sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)
\end{align*}
			
\paragraph{There are no samples in range:}
Now, consider the case $\cS^*_v = \emptyset$, then we claim $Y_v^\top \cup Y_v^\bot = Y_v^*$. Indeed, fix $\cS^*_{p(v)}$ (where $p(v)$ denotes the parent of $v$), and let
$q$ be the largest exponent of $2$ such that $q \leq |\cS^*_{p(v)}|-1$. Now enumerate $\cS^*_{p(v)} := \{ S_j, S_{j+1},\ldots,S_{j+p} \}$ for some $p < 2q-1$. Then $Y_v^\top = [S_{j+p-q},S_{j+p}]$ and $Y_v^\bot = [S_{j},S_{j+q}]$. Overall, $Y_v^\top \cup Y_v^\bot = [S_j,S_{j+p}] = Y_v^*$.

We conclude:
	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) \geq \LIS(X_v,Y_v^*)$$
	
This concludes the proof.

\end{proof}

%The argument is as follows:
%Consider a node $v_{r,i}$ in the tree. Suppose for a set of $j$s $J$ the $\LIS(X_i^r,\cup_{j \in J} Y_{i,j}) = l_{r,i,J}$. 
%Then whp, $\sum_{r'\leq r,j \in J} l_{r',i',j} \geq l_{r,i',j}$, with the additional requirement that for a fixed $r'$ the $j$s are coherent and all $v_{i',j}$ are descendants of $v_{r,i}$.



==> proof_of_reslis_invariant.tex <==
\subsection{Proof of \Cref{lm::reslis_invariants_new}}

We will use the following tail bounds for sums of independent geometric random variables, which are special cases of results proved by~\cite{Janson18}.
\begin{theorem}[Theorems 2.1 and 3.1 in~\cite{Janson18}] \label{thm:janson_geometric_tail}
	Let $p \in (0,1]$, and $\bX_1,\cdots, \bX_m$ be independent \emph{Geometric}\hspace{0.04cm}$(p)$ random variables. Let $\bX = \sum_{i\in [m]} \bX_i$ and $\mu = \bE[\bX] = m/p$. Then for any $\alpha \in (0,1)$, we have 
	\[
		\Pr\big[X \notin [(1-\alpha)\mu, (1 +\alpha)\mu]\big] \leq 2 \exp\left({-p \mu (\alpha - \ln (1+\alpha)}\right).
	\]
\end{theorem}
Note that $\alpha - \ln (1+\alpha) \geq 0$ for all $\alpha \in (0,1)$, with equality only at $\alpha = 0$. We first derive a simpler expression for the tail bounds, using the following claim:
\begin{claim} \label{clm:Janson_simple}
	Let $f : (-1,\infty) \rightarrow \R$ be defined as
	$
	f(x) = x - \ln (1+x).
	$
	The following  properties hold:
(i) $f(0) = 0$; (ii) $f(x) > x^2/4$ for all $x \in (-1,1]  \setminus \{0\}$; and
(iii) $f(x) \geq x/4$ for all $x \geq 1$.\snote{Note to self: Probably don't need the third property; check and remove.}
\end{claim}
\begin{proof}
	The claim follows from elementary calculus. For item (ii) it can be shown that  $g(x) = f(x) - x^2/4$ attains its minimum value $0$ at $x = 0$ and is strictly convex in $(-1,1]$. For item (iii) it is easy to verify that $h(x) = f(x) - x/4$ satisfies $h'(x) > 0$ for all $x \geq 1$, and hence its minimum value is $h(1) \geq 0.05$.
\end{proof}
%Letting $x = \lambda - 1$ in~\Cref{thm:janson_geometric_tail}, this claim allows us to replace the $\lambda - 1 - \ln \lambda$ term in the exponent of the tail bounds by either $(\lambda-1)^2 / 4$ or $(\lambda-1)/4$, depending on whether $\lambda < 2$ or $\lambda \geq 2$.

\begin{proofof}{\Cref{lm::reslis_invariants_new}}
We now prove each invariant stated in the lemma.\snote{Note to self: Change $X \cap Y^{-1}$ to $y(X) \cap Y$ everywhere.}
\begin{enumerate}
    \item Each element of $X \cap Y^{-1}$ is sampled with probability
    \[
    p := \frac{b \log n}{|X \cap Y^{-1}|}.
    \]
    Fix a node $v \in V$, and let $r_v$ be the corresponding interval length. Then, we observe that $|X_v \cap Y^{-1}|$ is a sum of $r_v \log n$ independent Geometric$(p)$ random variables.\snote{Does this require more explanation?} So, we have
    \[
        \mu := \E\left[\left|X_v \cap Y^{-1}\right|\right] = \frac{r_v \log n}{p} = \frac{r_v}{b} \left|X \cap Y^{-1}\right|.
    \]
    Now, applying \Cref{thm:janson_geometric_tail} with $p,\mu$ as above and $\alpha = 0.1$, we have
    \[
        \Pr\left[\left|X_v \cap Y^{-1}\right| \notin \left[\frac{0.9 r_v}{b} \left|X \cap Y^{-1}\right|, \frac{1.1 r_v}{b}\left|X \cap Y^{-1}\right|\right]\right] \leq \exp(-\Omega(p \mu)) = \exp(-\Omega(r_v \log n)) \leq \frac{1}{n^3},
    \]
    by choosing a sufficiently large constant in the  sampling rate.\snote{Make sure the algorithm does this.} Using a union bound over all $v \in V$, we conclude that Item (1) holds with probability at least $1-1/n^2$. We assume that this invariant holds for the rest of the proof.
    
    \item Each element in $X_v \cap Y{-1}$ is sampled with probability
    \[
        p':= \frac{r \log n}{|X_v \cap Y^{-1}|}.
    \]
    For for each $j \in [r-1]$, $|X_v \cap Y_{v,j}^{-1}|$ \blue{(equivalently, $|y(X_v) \cap Y_{v,j}|$)}\snote{Only holds if all elements distinct} is a sum of $\log n$ independent Geometric($p'$) random variables. So,
    \[
        \mu':= \E\left[\left|X_v \cap Y_{v,j}^{-1}\right|\right] = \frac{\log n}{p'} = \frac{|X_v \cap Y^{-1}|}{r_v} \in \left[\frac{0.9}{b} \left|X \cap Y^{-1}\right|, \frac{1.1}{b} \left|X \cap Y^{-1}\right|\right],
    \]
    where we have used the previous invariant to bound $\mu'$. Again we invoke \Cref{thm:janson_geometric_tail} with $p',\mu'$ as above and $\alpha = 0.1$ to get that with probability at least $1-1/n^3$,
    \[
    \left|X_v \cap Y_{v,j}^{-1}\right| \in [0.9\mu', 1.1\mu'] \subset \left[\frac{0.81}{b} \left|X \cap Y^{-1}\right|, \frac{1.21}{b}\left|X \cap Y^{-1}\right|\right].
    \]
    
    \item \snote{This is proof of \Cref{lm::reslis_invariants}, item 3; need to edit notation and paste there.} Fix $r \in 2^{[\log (1/\lambda)]}$. Consider a coherent set $\{(i,Y^r_{i,j(i)}\}_{i \in [b/r]}$, where for each $i \in [b/r]$, there is at most one $j=j(i)\in [r-1]$ such that $Y^r_{i,j(i)}$ is part of the set.\snote{The lemma statement needs to specify that $j$ is a function of $i$.} Then by definition of a coherent set and the order relation over intervals, we have $i_1 < i_2 \equiv \max(Y^r_{i_1,j(i_1)}) < \min(Y^r_{i_2,j(i_2)})$. For each $i \in [b/r]$, let $\cL_i$ be the longest increasing sequence in $X_i$\footnote{We choose one sequence arbitrarily if there are multiple longest increasing sequences.}, with values restricted to $Y^r_{i,j(i)}$. $\LIS(X_i, Y^r_{i,j(i)})$. By the property of coherence and the fact that $Y^r_{i,j(i)}) \subset Y$ for all $i$, the sequence $\cL = \cup_i \cL_i$ is clearly a valid increasing subsequence of $X$ with values restricted to $Y$. As this subsequence has length $\sum_i \LIS(X_i, Y^r_{i,j(i)})$, we conclude that $\sum_i \LIS(X_i, Y^r_{i,j(i)}) \leq \LIS(X,Y)$.
    
\end{enumerate}
    
\end{proofof}

==> pseudo.tex <==
\section{Algorithm for finding multiple $\LIS$}

\begin{theorem}
Consider an instance $\cE$
\end{theorem}

\subsection{Old}

\aanote{TO REMOVE?}

We note that a brute force search for $\LIS$ will take $O(n\cdot k^2 / \lambda)$ time, which is prohibitive for our fine-grained application. We hence devise the following parallel $\LIS$ approximation algorithm.

We call the below initially with $U = [n] \times [k]$ and iterate it with all $\lambda' \in 1/E_2(1/\lambda)$.

\blue{Intuition: The idea is that if there are many disjoint (non-overlapping) pseudo solutions of a certain range, there are many combinations as well, then splitting them into buckets we can still find pseudo solutions with almost same length, hence we never have to brute force too many (i think $\log(nk)$ overhead only)}
\newcommand{\fs}{\textsc{Finding-Solutions}}
\subsection{Algorithm Description}
\paragraph{\fs($g,U,\lambda$)}
\begin{enumerate}
    \item If $|U| \leq O(n \log^{O(1)}(nk))$, compute and return all solutions of length at least $\lambda n$ in $U'$ using the algorithm in \cite{rubinstein2019approximation}.
    \item Let $U_1, U_2$ be an iid coin-flip partition of $U$.
    \item $\cS_1 \gets \textsc{Finding-Solutions}(g,U_1,\lambda(1-\delta))$.
    \item $\cS_2 \gets \textsc{Finding-Solutions}(g,U_2,\lambda(1-\delta))$.
    \item $U' \gets U \setminus (\cS_1 \cup \cS_2$).
   % \begin{enumerate}
        \item Compute $\polylog(nk)$ solutions of length at least $\lambda n$ in $U'$ using the algorithm in \cite{rubinstein2019approximation}; let $\cS'$ be this set of such solutions.
        \item If there are no more solutions left, return $\cS' \cup \cS_1 \cup \cS_2$.
        
%        \item If $|\cS_1 \cup \cS_2| > |U|/\Theta(\polylog nk)$, return $\cS_1 \cup \cS_2 \cup \textsc{Finding-Solutions}(g,U',\lambda)$.    
\item Otherwise, return $\cS_1 \cup \cS_2 \cup \cS' \cup \textsc{Finding-Solutions}(g,U' \setminus \cS',\lambda)$.
        %If there are any 
        %\nnote{we may need to stop after $\log (nk)$ solutio%ns are found, then find the rest at the next $\lambda$ for some extremal cases...}.
  %      \item return $\cS' \cup \cS_1 \cup \cS_2$.
  %  \end{enumerate}
    
\end{enumerate}

\subsection{Correctness}

\begin{claim}
    Let $p \subset U$ be a solution. Then at least one of $U_1$ and $U_2$ contains an increasing subsequence of $p$ of length at least at least $|p|/2$.
\end{claim}

\begin{proof}
    This is immediate from the fact that $\{U_1,U_2\}$ is a partition of $U$.
\end{proof}

\begin{corollary}
    The recursion depth of $\fs$ is at most $O(\polylog (nk))$
\end{corollary}

\begin{claim}
    Suppose any (balanced?) set of coordinates $U$ has at least $s$ disjoint solutions of length $\geq|p|$. Then if we subsample $\tilde{U}$ with probability $q > 1/3$, we find w.h.p  $q(1-\delta)s$ disjoint solutions of length at least $\alpha|p|$, where $\alpha > 1-\tfrac{1}{\log nk}$.
\end{claim}

\subsection{Time complexity}


==> reslis.tex <==
%\newpage

\section{Algorithm for $\reslis$: Proof of Theorem~\ref{thm::sl_rec_tree}}\label{sec::reslis}
%\snote{Remove the newpage later.}

Here we present our construction for the $\reslis$ problem, and prove~\Cref{thm::sl_rec_tree}. %\snote{Should we restate the theorem here, or later when we prove it? I tried to put it here but it is quite a long statement and seems unwieldy.}
Recall that we are given an interval $X \subset [n]$, a sequence %input
$y \in \N^{X \times [k]}$ and a range of values %value range
$Y \subset \N$, and the goal is to approximate $\blocklis(y,X,Y)$, ie the length of a maximal sub-sequence $\OPT$, specified by %sub-sequence $(w_1, u_1), (w_2, u_2), \cdots, (w_\ell, u_\ell)$ such that:\snote{Check problem description}
a set of indeces $w_1,w_2,\ldots,w_\ell \subseteq X \times [k]$ such that:
\begin{itemize}
    \item The first coordinates $\{(w_i)_1\}_{i \in [\ell]}$ are disjoint.
    \item The set of (first coordinate,value) pairs $\{((w_i)_1,y_{w_i})\}_{i \in [\ell]} \subseteq X \times Y$ and is a coherent set.
    \item $|\OPT|$ is of maximal length.
\end{itemize}
%\begin{itemize}
%    \item $1 \leq w_1 < w_2 < \cdots < w_\ell \leq |X|$,
%    \item $u_i \in [k]$ and $y_{u_i, w_i} \in Y$ for all $i \in [\ell]$, and
%    \item the sequence $(y_{w_1, u_1}, y_{w_2, u_2)}, \cdots, y_{w_\ell, u_\ell})$ is increasing.
%\end{itemize}%$\OPT \triangleq \{(w,y_w)\}_w
%such that $(w_1,y_w)$ is monotone, and all $y$-values in the subsequence are in $Y$.

Our construction, at high-level, will break-down the $\reslis$ problem above to a  $\genlis$ instance over $|X|/r$ blocks. While the first coordinates of each block values can be computed directly, each genuity flag will be defined as a  $\blocklis$ instance of a block interval of some smaller size $r$. Intuitively, one can think of the $\genlis$ instance as solving the {\em global $\LIS$}, while each $\reslis$ instance is solving {\em local $\LIS$}, over multiple value ranges. Overall, we will show such formulation is equivallent to a composition of functions, and use the tree decomposition Lemma to obtain our correctness and complexity guarantees.

\subsection{\genlis Extension}
%Before Proving Thm~\ref{thm::sl_rec_tree}
Before describing our construction for proving~\Cref{thm::sl_rec_tree}, we first introduce a slightly stronger version of it, which will be easier for us to work with. In particular, we introduce 2 relaxations for the \genlis algorithm requirements. First, we allow the inputs to be blocks of {\em intervals} rather than integers, and second, we require the approximation to improve if most blocks are empty. Those relaxation are needed as part of the overall setup, as was described in the Technical Overview\nnote{make sure we explain the setup in TO}. Overall, the stronger version is the following:

\begin{lemma}[Thm~\ref{thm::sl_rec_tree}, stronger] \label{lm::sl_rec_relaxed}
Fix input $y \in \N^{n \times k}$, a block interval $X$, value range interval $Y \subseteq \N$, and parameters $\lambda \in (0,1)$, $\tau \in E_2(n)$, and $t \in \N$%\nnote{explain what each of these mean}
. Fix monotone functions $a_g,c_g :  %on $
\R_+ \rightarrow \R_+$ and $a_s,c_s:\R^3_+ \rightarrow \R_+$. Suppose there exist the following algorithms:

\begin{enumerate}
\item[$\cA_{GL}$:] Fix $\genlis_{n_g,k_g}$ instance $g \in (\cI \times \zo)^{k_g \times n_g}$. %\snote{$k_g \times n_g$?}
Fix $\eta > 1/k_g$ such that $g$ has at most $\eta n$ non-empty blocks. 
Then, given parameter $\lambda_g$ and \prectree $T_{1/c_g(\lambda_g)}(g)$, $\cA_{GL}$ outputs  $\left(a_g\left(\tfrac{\lambda_g}{\eta k_g}\right),\lambda_g n_g\right)$-approximation to $\genlis(g)$ in time $t_{GL} = \tO(\eta \cdot n_g \cdot k_g)$ w.h.p.%\nnote{define $\eta$} %_{n_g,k_g}
\item[$\cA_{BL}$:] For any interval $X' \subset X$ and value range $Y' \subset Y$, and any $\lambda_s < 1$,\nnote{add the $\tau$ part in the proof...} %\nnote{say something about the sizes of inputs / $k$. In particular, show they decay with rate $n^\epsilon$ to converge in constant steps to composition of constant $\genlis$ instances}, 
given a \prectree $T_{1/c_s(|X'|,\tau,\lambda_s)}(y(X'))$, outputs $\left(\alpha_s,\lambda_s |X'|\right)$-approximation to $\blocklis(y,X',Y')$  w.h.p., where $\alpha_s \triangleq a_s\left(|X'|,\tau,\tfrac{\lambda_s |X'|}{|y(X') \cap Y'|}\right)$. The run-time $t_{BL}$ is at most $t \cdot c_s(|X'|,\tau,\lambda_s)$.
\end{enumerate}
%\paragraph{$\cA_{GL}$:} Given $\genlis_{k_g}$ instance $g$ and \prectree $T_{c_g(\lambda_g)}(g)$, output w.h.p. $(a_g(\lambda_g/k_g),\lambda_g n_g)$-approximation for $\genlis_{k_g}(g)$.

%\paragraph{$\cA_{RL}$:} For any pair of intervals $X' \subseteq X$ and $Y' \subseteq Y$\nnote{say something about the sizes of inputs / $k$}, letting $\alpha_s \triangleq a_s\left(\tfrac{\lambda_s |X'|}{|y(X') \cap Y'|}\right)$; if given a \prectree $T_{c_s(\lambda_s)}(y(X'))$, output w.h.p. $\left(\alpha_s,\lambda_s |X'|\right)$-approximation for $\LIS_{k}(X',Y')$.

	 Then, for $c>1$, given a \prectree $T_{1/c}(y)$, % access to $y(X)$,
	 we can produce a $(\alpha, \lambda |X|)$-approximation for $\blocklis(y,X,Y)$ w.h.p., where $c,\alpha$ are such that, for all $\lambda_s, \lambda_g \in [\lambda,1]$, $k_g \in [1,1/\lambda]$ satisfying $\tfrac{\lambda_s \lambda_g}{k_g} = \Omega(\lambda
	 \log 1/\lambda)$:
	\begin{itemize}
	\item
$\alpha \ge \polylog (k/\lambda) \cdot a_g(\lambda_g/k_g) \cdot a_s\left(\frac{|X|}{\tau},\tau,\tfrac{\lambda_s\cdot |X|}{|y(X) \cap Y|}\right)$,
\item
$c \ge  \polylog (n) \cdot \left(\tau / \lambda + c_g(\lambda_g) \cdot c_s\left(\frac{|X|}{\tau},\tau,\lambda_s\right)\right)$ .
	\end{itemize}
	The algorithm's run-time is $\tO\left(\tau k/\lambda + |X|^{o(1)} \cdot % \tfrac{
	c %}{ c_s(|X'|,\tau,\lambda_s)\nnote{that might not be true look later...}} 
	\cdot t\right)$.%$|X|^{o(\log_\tau(|X|)} \cdot c$.
\end{lemma}

To prove Thm~\ref{thm::sl_rec_tree}, we use the following reduction:

\begin{lemma}\label{lm::genlis_int_reduction}
    If there exists an algorithm $\cA$ that $(f(\lambda/k),\lambda n)$-approximates $\genlis_{n,k}$ for some function $f$ in time $t(n \cdot k)$ over integers, then there exists an algorithm $\cA'$ that $(O(f(\lambda/\eta k) \log(1/\lambda)),\lambda n)$-approximates $\genlis_{n,k}$ over intervals, where $(1-\eta) n$ fraction of blocks are empty (ie, contain 0 intervals). The run-time is $t(\eta n k) + O(n + \eta nk \log (\eta nk))$.
\end{lemma}

The proof of Lemma~\ref{lm::genlis_int_reduction} is deferred to Appendix~\ref{sec:genlis_ext}.

\begin{proof}[Proof of Theorem~\ref{thm::sl_rec_tree} using Lemma~\ref{lm::sl_rec_relaxed} and Lemma~\ref{lm::genlis_int_reduction}]
The proof is immediate since the relaxed algorithm assumption of Lemma~\ref{lm::sl_rec_relaxed} reduces to the stronger version using Lemma~\ref{lm::genlis_int_reduction}, with $O(\log 1/\lambda_g)$ extra approximation, which is contained in the $\polylog (k/\lambda)$ approx of parameter $\alpha$, and noting the additive time $O(n + \eta n_g k_g \log (\eta n_g k_g))$, can be contained in $\tO(\eta n_g k_g)$, as long as $\eta < 1/k$
\end{proof}

The rest of this section is devoted for proving Lemma~\ref{lm::sl_rec_relaxed}.
\input{reslis_algo_new}



\subsection{%Algorithm
Analysis}\label{sec::reslis_analysis}

\ssnote{State the actual bound on the output of the \reslis algorithm, i.e., \\$\widehat{L} \in \left[\reslis(y,X,Y) \cdot \lambda^{o(1)}- \lambda |y \cap Y|, \reslis(y,X,Y) \right]$ (not just in terms of functions $a_g$ etc.). Maybe state it as a a corollary of Theorem 5.2. Specify the exact expression hidden in $\lambda^{o(1)}$?}

Before analyzing the estimator $\widehat{L}$, we show several important properties. First, we claim that partitioning %a partition of
$X$ into intervals of smaller size %smaller size-intervals
and matching each one with a $Y$ range coherently cannot over-estimate the overall $\LIS$:

\begin{lemma}\label{lm::blis_upper}
	Fix an interval $Y \subset \N$. Let $X_1,\ldots,X_\ell$ be a partition of $X$ into consecutive, disjoint, in-order block intervals (i.e., $X_1 \prec X_2 \prec \ldots \prec X_\ell$) and let $\{(i,Y_i)\}_{i \in [\ell]}$ %\snote{$i \in [\ell]$}\nnote{yes}
	be an arbitrary {\em coherent} set. Then, we have $\sum_i \blocklis(y,X_i,Y_i \cap Y) \leq \blocklis(y,X,Y)$.%\snote{Are we allowing multiple $y$-intervals per block here?}\nnote{Note this has nothing to do with the construction, this is a general statement about coherency, ie that the "longest path" is at least the sum of local "longest-paths" where the $x$s and $y$s are coherent... of course, this will be true if $Y_i$s are not purely an intervals as well, as long as all its values are coherent with all other values in all other blocks, but thats irrelevant for the statement, as (in the implementation) we assume it is an interval here.}
\end{lemma}
\begin{proof}
%Let $l_i \triangleq  \blocklis(y,X_i,Y_i \cap Y)$ and let 
For each $i \in [\ell]$, let $\OPT_i \subseteq (X_i,*) \cap y^{-1}(Y_i \cap Y)$ be a set of coordinates of an optimal increasing subsequence for $\blocklis(y,X_i,Y_i \cap Y)$. %such that $(Q^*_{i,1},y(Q^*_i))$ forms an increasing subsequence of length $l_i$. 
Then $\sum_i |\OPT_i| %= \sum_i l_i 
= \sum_i \blocklis(y,X_i,Y_i \cap Y)$. On the other hand, since  $\{(i,Y_i)\}_{i \in [\ell]}$ is a coherent set, we have $y(p) \prec y(q)$ for any $p \in \OPT_i, q \in \OPT_j$ with $i < j$. We conclude that %obtain
the sequence $\cup_i \, y(\OPT_i) \subseteq Y$ forms an increasing subsequence of $y(X)$ of length $\sum_i \blocklis(y,X_i,Y_i \cap Y)$ %in $y(X)$
and the claim follows.
%	\snote{Edit notation.} Fix $r \in 2^{[\log (1/\lambda)]}$. Consider a coherent set $\{(i,Y^r_{i,j(i)}\}_{i \in [b/r]}$, where for each $i \in [b/r]$, there is at most one $j=j(i)\in [r-1]$ such that $Y^r_{i,j(i)}$ is part of the set.\snote{The lemma statement needs to specify that $j$ is a function of $i$.} Then by definition of a coherent set and the order relation over intervals, we have $i_1 < i_2 \equiv \max(Y^r_{i_1,j(i_1)}) < \min(Y^r_{i_2,j(i_2)})$. For each $i \in [b/r]$, let $\cL_i$ be the longest increasing sequence in $X_i$\footnote{We choose one sequence arbitrarily if there are multiple longest increasing sequences.}, with values restricted to $Y^r_{i,j(i)}$. $\LIS(X_i, Y^r_{i,j(i)})$. By the property of coherence and the fact that $Y^r_{i,j(i)}) \subset Y$ for all $i$, the sequence $\cL = \cup_i \cL_i$ is clearly a valid increasing subsequence of $X$ with values restricted to $Y$. As this subsequence has length $\sum_i \LIS(X_i, Y^r_{i,j(i)})$, we conclude that $\sum_i \LIS(X_i, Y^r_{i,j(i)}) \leq \LIS(X,Y)$.
\end{proof}

Second, we argue two essential invariants of our construction, which will be used later to lower bound our estimator:

\begin{lemma}\label{lm::reslis_invariants_tree}
    Fix input $X,Y, y$. With high probability, %W.h.p.,
    all the following invariants hold for the $\reslis$ algorithm:%\snote{Specify high probability. Is it $1 - 1/n^2$?}
    \begin{enumerate}
    %	\item For all $r,i$: $|y(X^r_i) \cap Y| \in [0.9,1.1]\tfrac{rk|y \cap Y|}{b}$\nnote{Remove item (1).}.

    	\item Let $X^\chi = \left\{w \in X \mid |y_w \cap Y| \in [0.5,1] \chi\right\}$ and let $X^{r,\chi}_i = \left\{w \in X^{r}_i \mid |y_w \cap Y| \in [0.5,1] \chi\right\}$. For all $r,\chi,i$ and all $Y' \in \cY_i^{r,\chi}$, we have:\snote{Check the factor in blue here. Should it not depend on the radius of $x$-intervals?} 
    	\[
    	|y(X^{r,\chi}_i) \cap Y'| \leq \blue{\tfrac{1.1}{b}} \cdot |y(X^\chi) \cap Y|.
    	\]%\nnote{maybe change to $\tfrac{2.2\chi}{b}|X|$ bound instead...}.$$ 
    	 
		\item For all $r, \chi, i$, there exist sets of candidate intervals %interval sets 
		$\widetilde{\cY^{r,\chi}_i} \subseteq \cY^{r,\chi}_i$ such that:
		\begin{enumerate}[(i)]
		    \item $|\widetilde{\cY^{r,\chi}_i}| \leq 3$;
		    \item For all $r, \chi$: $\{(i,\cup_{Y \in \widetilde{\cY^{r,\chi}_i}} Y)\}_{i}$ is a coherent set; and 
		
    		\item \[
		    \sum_r \sum_\chi \sum_i \sum_{Y' \in \widetilde{\cY^{r,\chi}_i}}\LIS(X^r_i,Y') \geq \LIS(X,Y) - 5\lambda |X|.
    		\]
    	\end{enumerate}
    \end{enumerate}
\end{lemma}

%We prove Lemma~\ref{lm::reslis_invariants_tree} in Section~\ref{sec::resinv_proof}. 
%We now analyze the correctness %and complexity 
%of our algorithm, proving Theorem~\ref{thm::sl_rec_tree}:

We analyze the correctness and complexity of our algorithm, proving \Cref{thm::sl_rec_tree} assuming \Cref{lm::reslis_invariants_tree}, in \Cref{sec:proof_thm_5.2}. We prove \Cref{lm::reslis_invariants_tree} in \Cref{sec::resinv_proof}. 

\subsubsection{Proof of \Cref{thm::sl_rec_tree} using \Cref{lm::reslis_invariants_tree}} \label{sec:proof_thm_5.2}

%\begin{proof}[Proof of Theorem~\ref{thm::sl_rec_tree} using Lemma~\ref{lm::reslis_invariants_tree}]

%\ns{adapt to new settings...}

%	\ns{fix/polish using new defs / invariants...}
	
%	Let $\ell^r_{i,j} \triangleq \LIS(X^r_i,Y^r_{i,j})$. 

	For all $r,i$ and all $Y' \in \cY^r_i$, let $\ell^{r}_{i,Y'} \triangleq \LIS(X^{r}_i,Y')$. 
	By Lemma~\ref{lm::reslis_invariants_tree} (2), we have that for some $r^*$ and $\chi^*$, there exists a coherent set of pairs 
	$P_{r^*,\chi^*} \subseteq \{(i,Y')\}_{i, Y' \in \widetilde{\cY^{r^*,\chi^*}_i}}$\snote{Can we write $P_{r^*,\chi^*} \subseteq \cup_i \{i\} \times \widetilde{\cY^{r^*,\chi^*}_i}$? I don't see the point of writing $P \subset \{a\}_{a \in A}$ rather than $P \subset A$.} such that:
	
	$$\sum_{(i,Y') \in P_{r^*,\chi^*}} \ell^{r^*}_{i,Y'} \geq \tfrac{\LIS(X,Y) - 5 \lambda |X|}{3\log (1/\lambda) \cdot \log(k)} > \tfrac{\LIS(X,Y) - 5 \lambda |X|}{3\log^2 (k/\lambda)}$$
	
%	\ns{here...}
	
	Now we introduce more notation. %$\ell^{r,\rho}_{i,Y'} \triangleq \LIS(X^{r,\rho}_i,Y') $ to be the lis, restricted to blocks with $[0.5,1]\rho$ elements in $Y'$\nnote{formalize}. 
	Let $P_{r,\chi,\rho} \triangleq \left\{(i,Y') \in P_{r,\chi} \mid |\cY^{r,\chi}_i| \in [0.5,1]\rho\right\}$, and let $\ell^*_{i,Y'}\triangleq \ell^{r^*}_{i,Y'}$. %Let $\kappa^* \triangleq \kappa_{t^*} = \tfrac{|X|}{bt^*}$.
	For any $\alpha_s > 1$, there must exist some $(t^*,\rho^*) \in E_2(1/\lambda) \times E_2(k)$ for which\footnote{Recall that $\kappa_{t^*} = r^*/t^*$.}
	\[
	\sum_{(i,Y') \in P_{r^*,\chi^*,\rho^*}} \1\left[\ell^*_{i,Y'} \geq %\tfrac{2a_s |X|}{bt^*}
	2\alpha_s \cdot \kappa_{t^*} \right] \geq \tfrac{1}{2\alpha_s \kappa_{t^*}} \cdot \tfrac{\LIS(X,Y) - 5\lambda|X|}{3\log^4 (k/\lambda)}
	\]%\log^2(1/\lambda)}\geq \tfrac{bt^*}{2a_s |X|} \cdot \tfrac{\LIS(X,Y) - 2.2\lambda|X|}{3\log^4 (k/\lambda)}$$
		
    Let us first argue correctness. Define $P^* \triangleq P_{r^*,\chi^*,\rho^*}$ and \blue{$\kappa^* \triangleq \kappa_{t^*} = \tfrac{r^*}{t^*}$}. %$\tfrac{|X|}{bt^*}$
    Also define \blue{$\eta = \eta(r^*)$} as the fraction of intervals %\snote{This was "blocks"} %blocks
    of radius $r^*$ \snote{I replaced all occurrences of $r$ here and in the next equation with $r^*$.}
    with $|\cY_i^{r^*}| \in [0.5,1]\rho^*$. Formally,
    \[
    \eta \triangleq \frac{|\{i \in [|X|/r^*]: |\cY_i^{r^*}| \in [0.5,1]\rho^*\}|}{|X|/r^*}.
    %\eta \triangleq \frac{|\{i \in [|X|/r]: |\cY_i^r| \in [0.5,1]\rho^*\}|}{|X|/r}.
    \]
    
Recall the following %statement
guarantees for each pair $(i,Y') \blue{\in P^*}$:
    \begin{enumerate}
        \item Let $\widehat{\ell^*_{i,Y'}}$ be the output of $\estreslis(X^{r^*}_i,Y',\tfrac{1}{t^*},\tau)$. %Since $\LIS(X^{r^*,\chi^*}_i,Y') \leq \LIS(X^{r^*}_i,Y')$, 
        Then $\widehat{\ell^*_{i,Y'}}$ is a %$\left(a_s\left(\tfrac{|X^{r^*}_i|}{t^*|y \cap Y'|}\right),\tfrac{|X_i^{r^*}|}{t^*}\right)$
        $\left(a_s\left(|X^{r^*}_i|, \tau, \tfrac{|X^{r^*}_i|}{t^*|y \cap Y'|}\right),\tfrac{|X_i^{r^*}|}{t^*}\right)$
        -approximation of $l_{i,Y'}^*$.\snote{Here $a_s$ was initially written 1 argument. I changed it - please check.}
        
        \item Let $\Lambda^* \triangleq \Lambda_{r^*,\chi^*,t^*,\rho^*}$. The output of $\estgenlis(\Lambda^*, \lambda t^*)$ is a $\left(a_g\left(\tfrac{\lambda t^*}{\eta \rho^*}\right) % \cdot \tfrac{|X|}{|y \cap Y|})
        , \tfrac{\lambda t^* |X|}{r^*}\right)$-approximation\snote{Changed the additive approximation given the new meaning of $r^*$.} of $\sum_{(i,Y') \in P^*} \1\left[\widehat{\ell^*_{i,Y'}} \geq \kappa^*\right]$.%\ns{We need roughly $b/\rho^*$ in the second term, which is OK since $\sum_i |\cY_i^r| = O(b \log (1/\lambda))$ for any $r$, just need to make it works well with the tree-decomposition Lemma...}
    \end{enumerate}
     
      %(assume for now the output of $\genlis(\Lambda^*, \lambda t^*)$ is a $(a_g(\lambda t^* / \rho^*) % \cdot \tfrac{|X|}{|y \cap Y|})
     %   ,\lambda t^* \cdot b/\rho^*)$-approximation. 
    
     Let $\alpha_s \triangleq a_s\left(r^*,\tau,\tfrac{2r^*}{t^*} \cdot \tfrac{b}{|y \cap Y|}\right)$ %$\alpha_s \triangleq a_s\left(\tfrac{|X|r^*}{b},\tau,\tfrac{2r^*}{t^*} \cdot \tfrac{|X|}{|y \cap Y|}\right)$ %(noting that $\tfrac{2r^*}{t^*} \cdot \tfrac{|X|}{|y \cap Y|} > \tfrac{|X^{r^*}_i|}{t^*|y \cap Y'|}$ for all $(i,Y') \in P^*$) 
     and $\alpha_g \triangleq a_g\left(\tfrac{\lambda t^*}{\eta \rho^*}\right)$. \snote{Please check the calculations in this paragraph. I have NOT updated the value of $r$ inside this red paragraph. The relation is: $r_{old} = r_{new}\cdot b/|X|$.}\red{We note that $\tfrac{2r^*}{t^*} \cdot \tfrac{\lambda t^*}{\eta \rho^*} = \tfrac{2 \lambda r^*}{\eta \rho^*}$\snote{There was an extra $2$ in numerator.}. To further analyze this quantity, observe that 
     \[
        \sum_i |\cY_i^{r^*}| \leq |p| \log \tfrac{1}{\lambda} = s \log \tfrac{1}{\lambda} = b \cdot \log \tfrac{1}{\lambda} \cdot O(\log n \log k).
     \]
     %$\sum_i |\cY_i^{r^*}| \leq |p| \log (1/\lambda)$, and
     \snote{I think the bounds here should be multiplied by $O(\log n \log k)$ because the number of sampled blocks $s = b O(\log n \log k)$; is that fine?}
     Hence the number of intervals $X_i^{r^*}$ where $|\cY_i^{r^*}| \geq \rho^*/2$ is at most $2b \log (1/\lambda)/\rho^*$. Hence $\eta b / r^* \leq 2b\log (1/\lambda)/\rho^*$ which implies $\eta \rho^* \leq 2r^* b\log (1/\lambda)$. So $2\lambda\tfrac{2r^*}{\eta \rho^*} \geq 4\lambda \log(1/\lambda)$ as needed.
     }
    % ...\ns{here...}
     
     %\ns{We need $\rho^* \leq r^*$, which is OK since $\sum_i |\cY_i^r| = O(b \log (1/\lambda))$ for any $r$, just need to make it works well with the tree-decomposition Lemma... To solve this, define the $\genlis$ problem where the number of elements per block is $k$ on average, and each one either 0 or some bigger number... and the approximation is using $k$ still... todo this once sandip is done with genlis...}
     
     We use the above bounds to obtain a lower bound on $ L^* \triangleq L_{r^*,\chi^*,t^*,\rho^*}$. Assuming $c > c_s \cdot c_g \cdot \polylog(n)$, we invoke Lemma~\ref{lm::tree_decomposition} to get that the quantity $L^*$ is a $(\alpha_g, 
    %\lambda t^* \cdot b}{r^*}
    \tfrac{\lambda |X| t^*}{r^*})$-approximation\snote{based on the new $r$, I updated this additive approximation here, and in the following steps.} of $\left(\alpha_s,\tfrac{|X_i^{r^*}|}{t^*}\right)$-local $\{\ell^*_{i,Y'}\}_{i,Y'}$ approximations. We therefore derive the following: 
    \begin{align*}
        L^* &\geq \left(\tfrac{1}{\alpha_g}\sum_{(i,Y') \in P^*} \1\left[\widehat{\ell^*_{i,Y'}} \geq \kappa^* \right] - \tfrac{\lambda |X| t^* }{r^*}  \right) \cdot 0.3 \kappa^* \\
        &\geq \sum_{(i,Y') \in P^*} \left(\tfrac{1}{\alpha_g}\1\left[\ell^{*}_{i,Y'} \geq \alpha_s\left(\kappa^* + \tfrac{|X_i^r|}{t^*}\right)\right] - \tfrac{\lambda |X| t^* }{r^*} \right) \cdot 0.3 \kappa^* \\
        &\geq \tfrac{0.3 \kappa^*}{\alpha_g} \cdot \sum_{(i,Y') \in P^*} \left(\1\left[\ell^{*}_{i,Y'} \geq \alpha_s\left(\kappa^* + \tfrac{r^*}{t^*}\right)\right]\right) - 0.3 \kappa^* \cdot \tfrac{\lambda |X| t^* }{r^*} \\
        &\geq \tfrac{0.3 \kappa^*}{\alpha_g} \cdot \sum_{(i,Y') \in P^*} \left(\1\left[\ell^{*}_{i,Y'} \geq \alpha_s\left(\kappa^* + \kappa^*\right)\right]\right) - 0.3 \lambda |X| \\
        &\geq \tfrac{0.3 \kappa^*}{\alpha_g} \cdot \tfrac{1}{2\alpha_s \kappa_{t^*}} \cdot \tfrac{\LIS(X,Y) - 5\lambda|X|}{3\log^4 (k/\lambda)}
 - 0.3 \lambda |X| \\
    &> \tfrac{1}{20 \cdot \alpha_s \alpha_g \log^4 (k/\lambda)} \cdot \LIS(X,Y) - \lambda |X|
    \end{align*}
    
   
    %\ns{check the connection between $\alpha_g$ and $\alpha_s$ to make sure is what we need}
    For the upper bound, we use Lemma~\ref{lm::blis_upper} to claim that for any set of parameters, and any choice of coherent pairs, $\widehat{L}$ is upper bounded by $\blocklis(y,X,Y)$, and hence any approximation of such quantity is guaranteed to be bounded by $\blocklis(y,X,Y)$ as well.

    This concludes the correctness proof. 
    
    For the analysis of runtime, we first sample at most $c$ blocks for each set of parameters, and invoke %we use
    Lemma~\ref{lm::tree_decomposition} with some parameter $c_s \leq c/c_g$.\snote{Specify what $c_s$ is exactly?} 
    By the Lemma, the time complexity is $t_{GL}(n_g k_g) + |X|^{o(1)} \cdot t_{BL} \cdot c_s \cdot c_g$. We note that\snote{I think there should be an additional $O(\log n \log k)$ factor in the number of candidate intervals}
    \[
    \eta \cdot n_g \cdot k_g \leq \sum_i |\cY_i^r| \leq b \cdot \log \frac{1}{\lambda} = \frac{\tau}{\lambda} \cdot  \log \frac{1}{\lambda}.%\cdot \log(1/\lambda) = \tau \cdot  \log(1/\lambda)/\lambda.
    \]
    Summing over all parameters, the runtime is $\tO(t_{GL}(\tau/\lambda)) + |X|^{o(1)} \cdot t_{BL} \cdot c$.
   % \ns{take care of the small extra additive factor (say, by adding another 2 factor in the denominator. Add complexity analysis. Add the extra constant to Theorem.}
    
   % \ns{Think if can get this down to $1+\eps$...}
%\end{proof}




%%%
%
% OLD STUFF
%
%%%

%    \begin{align*}
%        L^* &\geq \left(\tfrac{1}{a_g}\sum_{(i,Y') \in P^*} \1\left[\widehat{\ell^*_{i,Y'}} \geq \tfrac{|X|}{bt^*}\right] - \lambda b t^* \right) \cdot 0.3 \kappa_t \\
%        &\geq \sum_{(i,Y') \in P_{r^*}} \left(\tfrac{1}{a_g}\1\left[\ell^{r^*}_{i,Y'} \geq a_s\left(\tfrac{|y \cap Y|}{ bk^*} + \tfrac{|y \cap Y_{i,j}|}{k^*}\right)\right] - \lambda b k^* \right) \cdot 0.9 \tfrac{|y \cap Y|}{bk^*} \\
%        &\geq \tfrac{1}{a_g} \sum_{(i,Y') \in P_{r^*}} \1\left[\ell^{r^*}_{i,Y'} \geq \tfrac{a_s \cdot|y \cap Y|}{ bk^*} + \tfrac{1.1 a_s |y \cap Y|}{b k^*}\right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9 \lambda |y \cap Y| \\
%    &\geq \tfrac{1}{a_g}\sum_{(i,Y') \in P_{r^*}}\1\left[\ell^{r^*}_{i,Y'} \geq \tfrac{2.1a_s \cdot|y \cap Y|}{ bk^*} \right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
%    &\geq \tfrac{1}{a_g} \cdot  \tfrac{bk^*}{2.1a_s |Y \cap y|} \cdot \tfrac{\LIS(X,Y) - \lambda|Y \cap y|}{\log^2 1/\lambda} \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
%    &> \tfrac{1}{2.5 a_s a_g \log^2 1/\lambda} \cdot \LIS(X,Y) - \lambda |y \cap Y|
%    \end{align*}
%


%\begin{proof}[Proof of Theorem~\ref{thm::sl_rec_tree} using Lemma~\ref{lm::reslis_invariants_tree}]
%
%\ns{adapt to new settings...}
%
%%	\ns{fix/polish using new defs / invariants...}
%	
%%	Let $\ell^r_{i,j} \triangleq \LIS(X^r_i,Y^r_{i,j})$. 
%	For all $i$ and all $Y' \in \cY_i$, let $\ell^r_{i,Y'} \triangleq \LIS(X^r_i,Y')$. 
%	By Lemma~\ref{lm::reslis_invariants} (3), we have for some $r^*$ a coherent set of pairs $P_{r^*} \subseteq \{(i,Y')\}_{i, Y' \in \cY_i}$ such that:
%	$$\sum_{(i,Y') \in P_{r^*}} \ell^{r^*}_{i,Y'} \geq \tfrac{\LIS(X,Y) - 2.2 \lambda |Y \cap y|}{3\log 1/\lambda}$$
%	
%%	\ns{here...}
%	
%	Hence, fix $a_s > 1$. There must exists some $k^*$ for which:
%	
%	$$\sum_{(i,Y') \in P_{r^*}} \1[\ell^{r^*}_{i,Y'} \geq \tfrac{2a_s |y \cap Y|}{ bk^*}] \geq \tfrac{bk^*}{2a_s |Y \cap y|} \cdot \tfrac{\LIS(X,Y) - 2.2\lambda|Y \cap y|}{3\log^2 1/\lambda}$$
%	
%    Now, let us first argue correctness. Recall the following statement guarantees for each $(i,Y')$ pair:
%    \begin{enumerate}
%        \item Let $\widehat{\ell^{r^*}_{i,Y'}}$ be the output of $\reslis(X^{r^*}_i,Y',\tfrac{1}{k^*})$. Then $\widehat{\ell^{r^*}_{i,Y'}}$ is a $(a_s(\tfrac{1}{k^*}),\tfrac{|y \cap Y'|}{k^*})$-approximation for $l_{i,Y'}^{r^*}$.
%        \item The output of $\genlis(g_{r,k},k \lambda)$ is a $(a_g(\lambda k^*),\lambda b k^*)$-approximation for $\sum_{(i,Y') \in P_{r^*}} \1[\widehat{\ell^{r^*}_{i,Y'}} \geq \tfrac{|y \cap Y|}{bk^*}]$.
%    \end{enumerate}
%     
%     We use the above to derive the following lower bound on $ L_{r^*,k^*}$:
%    
%    \begin{align*}
%        L_{r^*,k^*} &\geq \left(\tfrac{1}{a_g}\sum_{(i,j) \in P_{r^*}} \1\left[\widehat{\ell^{r^*}_{i,Y'}} \geq \tfrac{|y \cap Y|}{bk^*}\right] - \lambda b k^* \right) \cdot 0.9 \tfrac{|y \cap Y|}{bk^*} \\
%        &\geq \sum_{(i,Y') \in P_{r^*}} \left(\tfrac{1}{a_g}\1\left[\ell^{r^*}_{i,Y'} \geq a_s\left(\tfrac{|y \cap Y|}{ bk^*} + \tfrac{|y \cap Y_{i,j}|}{k^*}\right)\right] - \lambda b k^* \right) \cdot 0.9 \tfrac{|y \cap Y|}{bk^*} \\
%        &\geq \tfrac{1}{a_g} \sum_{(i,Y') \in P_{r^*}} \1\left[\ell^{r^*}_{i,Y'} \geq \tfrac{a_s \cdot|y \cap Y|}{ bk^*} + \tfrac{1.1 a_s |y \cap Y|}{b k^*}\right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9 \lambda |y \cap Y| \\
%    &\geq \tfrac{1}{a_g}\sum_{(i,Y') \in P_{r^*}}\1\left[\ell^{r^*}_{i,Y'} \geq \tfrac{2.1a_s \cdot|y \cap Y|}{ bk^*} \right] \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
%    &\geq \tfrac{1}{a_g} \cdot  \tfrac{bk^*}{2.1a_s |Y \cap y|} \cdot \tfrac{\LIS(X,Y) - \lambda|Y \cap y|}{\log^2 1/\lambda} \cdot \tfrac{0.9|y \cap Y|}{bk^*} - 0.9\lambda |y \cap Y| \\
%    &> \tfrac{1}{2.5 a_s a_g \log^2 1/\lambda} \cdot \LIS(X,Y) - \lambda |y \cap Y|
%    \end{align*}
%    
%   % \ns{take care of the small extra additive factor (say, by adding another 2 factor in the denominator. Add complexity analysis. Add the extra constant to Theorem.}
%    
%   % \ns{Think if can get this down to $1+\eps$...}
%\end{proof}


==> reslis_algo.tex <==


\subsection{Algorithm}

The %$\reslis$ 
algorithm for the \reslis problem, named \estreslis, is described in Figure \ref{fig::ALG_reslis_amended}. %\Cref{fig::ALG_reslis_amended}.
%(Recall that $E_b(k) \triangleq \left\{b^i \mid i \in \{0,\ldots,\lfloor\log_b k\rfloor \}\right\}$.)

\subsubsection{Global \LIS vs. Local \LIS}
We first provide some intuition underlying the algorithm, and in particular, for {\em balancing} the  ``global \LIS'' and ``local \LIS'', a necessary ingredient of the \reslis algorithm. Suppose that $k = 1$, %and $\cE = \N$, 
so that the problem reduces to a standard $\LIS$ problem. \blue{In this special case, it might be useful to visualize the instance as a set of points on a standard two-dimensional grid, with $X$ being an interval on the $x$-axis, and the element $(i,y_i)$ being represented by the point with $x$-coordinate $i$ and $y$-coordinate $y_i$. In this equivalent formulation, the objective is to determine the maximum length of a subsequence that is increasing with respect to both axes.}

Assume further that a longest increasing subsequence $\OPT$ is of length approximately $\lambda |X|$. Note $\OPT$ can be distributed arbitrarily with respect to $X$. %$x$-positions. %, subject to the constraint that the sequence is increasing. 
%For instance, with respect to the position \blue{($x$-coordinate)}, if we divide 
Now, fix an optimal solution $\OPT$, choosing one arbitrarily if there are multiple optimal solutions. To approximate $\OPT$, we fix some length $r$, and use the standard, in-order partitioning of $X$ into $\ell = |X|/r$ mutually disjoint and covering intervals $X_1^r, \cdots, X_\ell^r$ of length $r$ each. There are two possible extreme scenarios for the distribution of $\OPT$:%Intuitively, one can consider the following extremes:

\begin{enumerate}
    \item $\OPT$ is uniformly distributed accross all intervals, i.e., each interval $X_i^r$ contributes approximately $\lambda r$ elements to $\OPT$.
    \item %There exists 
    All $\OPT$ coordinates belong to roughly $\lambda |X| / r$ intervals $X_i^r$, meaning that all elements in those intervals are part of the $\OPT$, and the other intervals do not contribute at all. %In such a case, the restriction of $\OPT$ to a small fraction of the intervals is very dense, and $\OPT$ is very sparse elsewhere.
    

\end{enumerate}

%\blue{We need to adopt different procedures to solve the problem in the two extreme cases above. 
Intuitively speaking, one can consider the problem of {\em certifying an alignment} harder if less elements participate in an alignment.
Therefore, in the first case above, one has to ``work harder'' on the global alignment to find the %candidate
participating intervals; however, little effort is required to verify the local \LIS in each interval of interest, i.e., to get a lower bound on the \LIS within each interval. %On the other hand, i
In the second case, on the other hand, it should be easier to determine the global alignment, but it is more difficult %and expensive 
to approximate the local \LIS (within each interval).
%\snote{In first case, we have to work very hard on the global alignment to find the candidate intervals but we have to work very little to verify the local LIS. Opposite for the other case.}
%\ns{perhaps build intuition of solving each such extreme?}

Of course, an optimal solution can lie anywhere between these extreme scenarios. However, one can %eventually 
show that there must exist some $t \in [1,1/\lambda]$, such that there are approximately $1/t$ fraction of %\blue{coherent} 
 intervals, each having approximately $\lambda t r$ ``local'' contribution to $\OPT$. %$\approx 1/t$ fraction of blocks must have $\approx \lambda t r$ ``local'' contribution to the $\OPT$. 
%Similarly, the structure can vary widely with respect to the $y$-values \ns{why is this sentence here?}.
%Moreover, this can happen at very different scales in different parts of the input. For example, a solution can look uniform at the highest level, in the sense that the contribution of each block $X_i$ to $\OPT$ is $\lambda r$, but within $X_i$, the solution can be highly non-uniform (with respect to both indexes and $y$-values). We need to capture all such possibilities with a small number of \emph{candidate solutions} \ns{I am not sure this sentence is important / helps understanding.} .

%To do this, we use partitioning, discretization over several parameters, and recursion, along with sampling.

%\paragraph{Discretization.} Our algorithm will perform exponential discretization over several parameters, and take the maximum over all quantities for each fixed set of parameters. We introduce these parameters next.%\snote{It's not clear to me what this notation $\chi$ : $|y_{i} \cap Y|$ means. Is it not enough to just state which parameter is being discretized?}\nnote{just would like to clarify the use of parameter $\chi$, along the rest of parameters...}

%\begin{enumerate}
%	\item[$r$:] represents the \emph{radius}, i.e., the number of blocks in each interval $X^r_i$.
%	\item[$\chi$:] represents the number of ``admissible" elements per block, i.e., the number of elements  in the range $|y_{i} \cap Y|$.
%	\item[$\rho$:] represents the number of candidate intervals $|\cY_i^r|$.
%	\item [$t$:] is defined such that the fraction of participating block intervals in the overall sequence is $1/t$. This parameter characterises the relation between the ``global'' and ``local'' \LIS. In particular, for the 2 extreme scenarios outlined above, the parameter $t$ would be $1/\lambda$ and $1$ respectively. %\blue{``global" vs ``local" length}\snote{Give examples of $t$ in the two extreme cases outlined above.}
%\end{enumerate}

\subsubsection{Algorithm Overview}

Now we consider the general $\reslis$ problem. Before describing the algorithm, we first set up some concepts and notation that will be used in the algorithm and its analysis. For the sake of clarity, this exposition will be somewhat simplified \ns{Do you mean the next statements are informal / overloading notation / etc?}.

Fix a \emph{radius} $r \in \N$. We introduce the following quantities, whose precise definitions are in Figure \ref{fig::ALG_reslis_amended}:

\begin{enumerate}
    \item[$X^r_i$:] %An $x$-axis interval.
    A sub-interval of $X$.\snote{This was "An $x$-axis interval."} We divide $X$ into $|X|/r$ disjoint consecutive intervals $X^r_i$, each consisting of $r$ blocks. \ns{Formally, we need to deal with $|X|$ not divisible by $r$, probably by padding $X$ with ``empty characters'' to a length power of 2}
    
    \item[$\cS^r_i$:] A set of $y$-elements, sampled pseudo-uniformly from $y(X^r_i) \cap Y$.\snote{Is "pseudo-uniform" defined earlier, in Section 4?} %, sampled by the algorithm.%(The sampling procedure is described in detail later.)\snote{Rewrite}
    
    \item [$\cY^r_i$:] A set of %element 
    intervals on the $y$-axis (denoted ``candidate intervals"), which are generated over\snote{This was "conceptually associated to"} %conceptually associated to}
    $X^r_i$ using the sampled set $\cS^r_i$ above.%, and which are generated using the sampled set $\cS^r_i$ above.
    %, whose properties are described later.
\end{enumerate}

We now describe the main components of our algorithm.

%\begin{enumerate}
%    \item \textbf
    \paragraph{Sampling.} 
The algorithm starts by simulating uniformly random blocks $(w_j, y_{w_j})$ and then choosing random $y$-elements in $Y$ among the sampled blocks.

    %\item \textbf
        \paragraph{Discretization.} The algorithm performs exponential discretization over the following parameters, and outputs the maximum over all quantities for each fixed set of parameters. %We introduce these parameters next.
    %\snote{It's not clear to me what this notation $\chi$ : $|y_{i} \cap Y|$ means. Is it not enough to just state which parameter is being discretized?}\nnote{just would like to clarify the use of parameter $\chi$, along the rest of parameters...}

\ns{there are plenty of parameters, and we need to use more unified notation, for example, $?_i$ should be for $r$-radius interval, $?_w$ for a block, etc... consider adding notation table?}

%\ns{also, whenever we specify the parameters below, we should perhaps specify its range of values we are discretizing upon...}

\begin{center}
 \begin{tabular}{||c c l||} 
 \hline
 Symbol & Range & Description\\ [0.5ex] 
 \hline\hline
 $r$ & $(|X|/b)   \cdot [1,1/\lambda]$  & \emph{radius}, i.e., number of blocks in each interval $X^r_i$\\ 
 \hline
 $\chi$ & $[1,k]$ & number of ``admissible" elements in a block $y_w$, i.e., $|y_{w} \cap Y|$\\
 \hline
 $\rho$ & $[1,k]$ & number of candidate intervals $|\cY_i^r|$\\
 \hline
 $t$ & $[1,1/\lambda]$ & inverse of fraction of intervals participating in $\OPT$ \\ %[1ex] 
 \hline
 $\cS^{r,\chi}_i$ & & subset of sampled blocks in $X^r_i$ containing $\approx \chi$ values in $Y$\\
 \hline
 $\cY^{r,\chi}_i$ & & candidate intervals generated over $X^r_i$ using samples $\cS^{r,\chi}_i$\\
 \hline
\end{tabular}
\end{center}

\snote{Where should the table go? What other parameters should be added?}
\begin{enumerate}
	\item[$r$:] represents the \emph{radius}, i.e., the number of blocks in each interval $X^r_i$.
	
	\item[$\chi$:] represents the number of ``admissible" elements in a block $y_w$, i.e., the number of elements  in the range $y_{w} \cap Y$.
	\item[$\rho$:] represents the number of candidate intervals $|\cY_i^r|$.
	\item [$t$:] represents the inverse of the fraction of intervals participating in $\OPT$. This parameter characterises the relation between the ``global'' and ``local'' \LIS. In particular, for the 2 extreme scenarios outlined above, the parameter $t$ would be $1/\lambda$ and $1$ respectively. %\blue{``global" vs ``local" length}\snote{Give examples of $t$ in the two extreme cases outlined above.}
\end{enumerate}

    \paragraph{Generation of Candidate Intervals.} For each choice of $r$ and $\chi$ and each interval $i \in [|X|/r]$ containing approximately $\chi$ many $y$-values in the given range $Y$, the algorithm uniformly samples $y$-values and uses them to construct \emph{candidate intervals} $\cY^{r,\chi}_i$ by invoking a subroutine called $\partition$ (see Figure \ref{fig::ALG_partition}).
    
    %\item \textbf
    \paragraph{Decomposition and Recursion.} The next step is to determine, for each choice of parameters $(r, \chi, \rho, t)$, the largest set of coherent candidate intervals $|\{(i,Y'): Y' \in \cY^{r,\chi}_i\}_i|$ such that each candidate interval has local $\LIS$ at least $r/t$.\snote{Check the threshold here and in the algorithm.} To do this, the algorithm recursively invokes the \reslis algorithm on each interval $X^r_i$, marking the intervals with a sufficiently long local LIS as ``genuine", and then solving a ``global" $\genlis$ problem over the intervals. Thus, the problem is formulated as a composition of a $\genlis$ problem over many smaller $\reslis$ problems, \blue{and the \prectree decomposition (Lemma~\ref{lm::tree_decomposition}) is used to answer this question.}\snote{Check last sentence.}
    
    %\item \textbf
    \paragraph{Output.} Finally, the algorithm returns the solution with the maximum value among all solutions for each choice of the parameters.
%\end{enumerate}

\subsubsection{Candidate Intervals}

Now we describe our construction of the candidate intervals $\cY^{r,\chi}_i$ using the sampled $y$-values $\cS^{r,\chi}_i$, for some fixed $r, \chi$ and $i$. The high-level goal, as in \cite{rubinstein2019approximation}, is to cover an optimal LIS solution using a small number of coherent interval sequences called \emph{pseudo-solutions}, so that the largest LIS within all pseudo-solutions would be a good approximation to the optimum. However, our construction is significantly more delicate, as we require the candidate intervals to possess the following additional properties:

\begin{enumerate}
    \item For each $Y' \in \cY^{r,\chi}_i$, $|y(X_i^r) \cap Y'|$ contains few elements.
    
    \item There exists a coherent set of candidate intervals $\{(i,Y'): Y' \in \cY_i^{r,\chi}\}_i$  such that the sum over all the ``local $\LIS$'' approximately matches the overall $\LIS$.
\end{enumerate}

To accomplish this objective, we define candidate intervals based on samples from a slightly larger interval $\cS^{2r,\chi}_{i/2}$, which is called the ``parent'' of $\cS_i^r$, and denoted by $\cS^p$. \blue{At a high level, for every radius $r$, we want a small set of candidate intervals for each sub-interval $i \in [|X|/r]$ that essentially capture the local LIS, and are coherent across $i$. (It turns out it is sufficient to take only $3$ candidate intervals for each sub-interval $i$.) We accomplish this efficiently by considering the parent candidate intervals which are of twice the size, and using the parent sample $\cS^p$ to cover the gaps between the candidate intervals.} To be more precise, we allow slightly overlapping candidate intervals with the following restrictions:% samples in a candidate interval from such larger \blue{radius}, as long as:
\begin{enumerate}
	\item  Each $Y' \in \cY_i^{r,\chi}$ must start and end with a sample in $\cS^p$.
	\item Each $Y' \in \cY_i^{r,\chi}$ can intersect $\cS_i^{r,\chi}$ only at the borders.%
	\item One of the following must hold:
	\begin{enumerate}
	    \item $Y'$ starts or ends with a sample in $\cS_i^{r,\chi}$, or %\blue{radius} is on (at least) one of the edges
	    \item the number of samples from $\cS^p$  in $Y'$ is a power of 2. %This guarantee ensures not too many candidate intervals.
	\end{enumerate}
\end{enumerate}

These restrictions allow us to bound the number of candidate intervals, while also being able to capture most of an optimal solution in their union; see \Cref{lm::reslis_invariants_tree} for the precise statement.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Algorithm Description}

The $\reslis$ algorithm is described in Figure \ref{fig::ALG_reslis_amended}. %\Cref{fig::ALG_reslis_amended}.
(Recall that $E_b(k) \triangleq \left\{b^i \mid i \in \{0,\ldots,\lfloor\log_b k\rfloor \}\right\}$.) It uses the following mechanisms:

\paragraph{Element-sampling.}
Recall that the $\blocklis(y,X,Y)$ problem allows for multiple elements per block. %\snote{Changed from "coordinate"}.
The algorithm starts by simulating uniformly random blocks and then choosing a random $y$-element in $Y$.\snote{This description sounds like we are sampling \emph{a single} $y$-element directly, after sampling $X$-blocks. Rephrase?}

\paragraph{Partitioning.}\snote{I don't think the formal guarantee of the PartitionY algorithm is explicitly stated anywhere.}
We partition both the $X$-blocks and $y$-elements as follows:

For blocks, we simply fix a radius $r$, and divide $X$ into $|X|/r$ disjoint consecutive intervals $X^r_i$, each consisting of $r$ blocks.%let each interval $X^r_i$ contain \blue{$r$} %$nr/b$
%consecutive blocks \blue{for some parameter $b$ which will be defined later.}%\nnote{$b$ is yet undefined} %Our algorithm will iterate over all $r$ ``scales'' and partition the blocks to $X_i^r$ elements for each radius $r$.

We also define the sets $\cS_i^r$ by associating the $y$-values of the sampled elements from above\snote{What does "from above" mean here?} with %to 
their respective $X_i^r$ intervals.


Lastly, for each block interval $X_i^r$, using $\cS_i^r$, we define multiple %$y$
candidate intervals of $y$-value range %intervals 
$\cY^r_i \triangleq \{Y^r_{i,j}\}_j$. %We define the candidate intervals using the sampled elements. %\ns{write more...}
%First, to allow for smooth reduction to $\genlis$, we pair only one $j$ for each $r,i$; in particular, a pseudo-solution will consist of (at most) 1 candidate interval $Y_{i,j}$ for each block $X_i$.% (to allow that, we analyze over multiple radii $r$). %(note this makes the invariants Lemma slightly more subtle (part 4 in particular)). 
%In order to force at most one candidate interval per block, we generate the $\genlis$ instance where each coordinate represent a $(X_i,Y_{i,j})$ pair: the $X_i$ are sorted in order, but the $Y_{i,j}$ are sorted in {\em descending order} (for a fixed $i$). This results ensures at most 1 element per $x$-block can participate in any $\genlis$ increasing subsequence. %(alternatively,  1 candidate interval per block can participate in a pseudo-solution). 
%To allow that, we make a few adjustments to how we define $x$ and $y$-intervals. First, we define $X_i$ over multiple radii, denoted $X_i^r$. Second, 
%\ns{edit the below...}
This part requires care to ensure the following invariants (which are formalized later in Section~\ref{sec::reslis_analysis}):
\begin{enumerate}
    \item For each $Y' \in \cY_i^r$, $|y(X_i^r) \cap Y'|$ contains few elements.
    \item There exists a coherent set of candidate intervals $\{(i,Y'): Y' \in \cY_i^r\}_i$ \snote{We use $Y'$ here but $Y'_i$ later in Lemma 7.1. I think it would be unclear to the reader whether the coherent set can contain multiple $(i,Y)$ for each $i$. Fix everywhere.} such that the sum over all the ``local $\LIS$'' approximately matches the overall $\LIS$.
\end{enumerate}

For that task, we define candidate intervals based on samples from a slightly larger interval %\blue{radius}
(referred to as $\cS^p$ for the ``parent'' of $\cS_i^r$). Then we allow slightly overlapping candidate intervals using the following restrictions:\snote{Should we not go into so much detail in the introduction?}% samples in a candidate interval from such larger \blue{radius}, as long as:
\begin{enumerate}
	\item  Each $Y' \in \cY_i^r$ must start and end with a sample in $\cS^p$.
	\item Each $Y' \in \cY_i^r$ can intersect $\cS_i^r$ only at the borders.%
	\item One of the following must hold: either (i) $Y'$ starts or ends with a sample in $\cS_i^r$; %\blue{radius} is on (at least) one of the edges, 
	or (ii) the number of samples from $\cS^p$  %samples
	in $Y'$ is a power of 2. %This guarantee ensures not too many candidate intervals.
\end{enumerate}

\paragraph{Discretization.} Our algorithm performs exponential discretization over several parameters, and takes the maximum over all quantities for each fixed set of parameters. The parameters are:%\snote{It's not clear to me what this notation $\chi$ : $|y_{i} \cap Y|$ means. Is it not enough to just state which parameter is being discretized?}\nnote{just would like to clarify the use of parameter $\chi$, along the rest of parameters...}

\begin{enumerate}
	\item Radius $r$: the number of blocks in each interval.
	\item Elements per block in range $\chi$: $|y_{i} \cap Y|$.
	\item Number of candidate intervals $\rho$: $|\cY_i^r|$. 
	\item Fraction of participating block intervals in the overall sequence $1/t$ (i.e., ``global'' vs ``local'' length)
\end{enumerate}

Each of the parameters can take $\lessapprox k/\lambda$ values, % in $\lessapprox k/\lambda$ range,
hence the total overhead %``overhead''
is $O(\log(k/\lambda))$.



\paragraph{Decomposition and Recursion.} 
Once we discretize over all the above parameters, for each quadruple $(r,\chi,t,\rho)$ we formulate the following question: %\snote{This was "quantity"}: 
{\em What is the largest set of coherent candidate intervals $|\{(i,Y'): Y' \in \cY^r_i\}_i|$ such that each candidate interval has local \blue{\reslis} $\LIS$\snote{Define local LIS formally.} at least $|X_i^r|/t$?}%\snote{Replace $Y'$ with $Y'_i$ everywhere?}

We formulate this problem as a composition of a $\genlis$ problem over many smaller $\reslis$ problems. %\snote{This was "Such formulation is defined a composition of a $\genlis$ problem over many ``smaller'' size $\reslis$ problems."}
We use the \prectree decomposition Lemma~\ref{lm::tree_decomposition} to answer this question.
%We now present our algorithm for $\reslis$:
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h!] 
\setstretch{1.2}
  \begin{algorithm}[H]
%\begin{algorithmic}[1]
    %\caption{\reslis}
    \caption{\estreslis}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{%intervals $X, 
		An input $y \in \N^{|X| \times k}$ consisting of $|X|$ blocks with $k$ elements each, value range $Y \subseteq \N$, \\
		additive error parameter $\lambda \in (1/n,1)$, branching parameter $\tau$\nnote{think of $\tau = n^\eps$},
		Precision-Tree $T=T_{1/c}(y)$%\snote{What does $y_*$ denote here?}
 }
		%\KwOut{A number $\widehat{L} \in \left[\LIS(X,Y) \cdot \lambda^{o(1)}- \lambda |y \cap Y|, \LIS(X,Y) \right]$.\snote{Write this as $\hat{L} \in [0, \LIS(X,Y)]$ here and state these bounds later. Also specify $\lambda^{o(1)}$.} \nnote{fix...}%\snote{Does this mean $1/\lambda^{o(1)}$?}\nnote{Yes!}
		\KwOut{An integer $\widehat{L} \in \left[0, \reslis(y,X,Y) \right]$.%\snote{Write this as $\hat{L} \in [0, \reslis(y,X,Y)]$ here and state these bounds later. Also specify $\lambda^{o(1)}$.}
		}

     \If{$|X| < c$}{\Return $\widehat{L} \gets \LIS(X,Y)$ through exact computation.}
     
     Let $W \triangleq \{w \in X \mid y_{w} \cap Y \neq \emptyset\}$. \\
     Let $S$ be a uniformly distributed set of blocks stored at the root of $T$ of size $\geq c$. \\
	 $\theta \gets \Pr_{w \in S}[w \in W]$\nnote{add data-structure to obtain that quickly};
	 $\zeta \gets O(\log n);$ $b \gets \tfrac{\theta \tau}{\lambda}$.\\ %\ns{I think $b = n^\eps$ suffices.} 
   % and $t \gets O_\epsilon(\polylog(1/\lambda)/\lambda)$.\\

    Simulate $s= \zeta \cdot O(\log k) \cdot b$ %pseudo-random elements 
    %$(w_1, q_1),(w_2, q_2), \cdots, (w_s, q_s)$
    blocks $(w_1, y_{w_1}), (w_2, y_{w_2}), \cdots, (w_s, y_{w_s})$  %$x$-
    uniformly from $W$ using $S$\nnote{add data-structure to obtain that quickly}.
    %from $y^{-1}(Y)$ 
   % by querying $T$\nnote{we need to adjust number of blocks and add data-structure to obtain that}.\\ %\nnote{explain}, %by {\em rejection sampling}, 
    %where $w_1 < w_2 < \cdots < w_s$.\\
    
    For $\chi \in E_{2}(k)$: $\{p^\chi_1,p^\chi_2,\ldots\} \gets \{ w_a \mid a \in [s], |y_{w_a} \cap Y| \in [0.5,1]\chi \}$ where $p^\chi_j < p^\chi_{j+1}$ for all $j$.\\%$p^\chi_1 < p^\chi_2 < \cdots$.\\   
%    $\cS \gets \{q_j \sim y_{p_j} \mid j \in \N\log n \}$ \\
    %for $i \i$
    % and each $q_i \in y_{w_i} \cap Y$.\\ 
        \For{$r \in E_2(\theta/\lambda) \cdot |X|/b$}{
     $X^r_1,\ldots,X^r_{|X|/r} \gets$ a partition of $X$ into $|X|/r$ %$b/r$ 
     consecutive intervals, each of length $r$ %$|X| \cdot r/b$
     blocks.\\%\snote{Replaced $n$ with $|X|$}\\
     \For{$\chi \in E_{2}(k)$}{
        \For{$i \in [|X|/r]$}{
   %      \eIf{$|p^\chi| < \zeta \tau$}{
    %     $L_{r,\chi,*,*} \gets \vec{0}$.}{
     
     $\cS^{r,\chi}_i \gets \{q_{j} \sim \uniform(y_{p^\chi_j} \cap Y) \mid j \in \zeta\N \wedge p^\chi_j \in X_i^r\}$.\snote{Added this loop over $i$ because the next 2 lines both involve $i$.}\\% for $i \in [|X|/r]$.\\
     
     %\snote{Check if $X_i^r$ here and in following lines should be $X_i^{r,\chi}$}
    % \nnote{consider poissonization to get uniformity... check if we need different sets}. \\
     
     $\cY_i^{r,\chi} \gets \textsc{\partition}(r,\chi,i)$.\\
     }
     % for $i \in [|X|/r]$.\\%$i \in [\tfrac{1}{r|X|}]$. \\%\nnote{here (not done yet)...} \\
     %$\{Y^r_{i,j}\}_{j\in [r-1]} \triangleq [\cS^r_i(j+1),\cS^r_i(j)]$ be the candidate intervals for block $i$ (again, in descending order).\nnote{we used decreased order to ``force'' the longest $\genlis$ having at most one $j$ for each $i$} \\
      \For{$(t,\rho) \in E_2(\theta/\lambda) \times E_2(k)$}{
      % $\kappa_t \gets \tfrac{|p^\chi|/\zeta}{bt}$. \\
       $\kappa_t \gets \tfrac{r}{t}$.\snote{Check parameter setting, given the new definition of $r$.}\\
       %Let $g_{r,t}(i,*) \triangleq [(Y',\1[\reslis(X^r_i,Y',\tfrac{1}{t},T_i^*\footnote{By $T_i^*$ we mean a Precision-Tree access to $X_i$ with sufficiently small parameter}) > \kappa_t])]_{Y' \in \cY_i^r}$. \\
        \For {$i \in [|X|/r]$}       
 %       \For {$\{i \in [|X|/r] \mid \left|\cY_i^{r,\chi}\right| \in [0.5,1]\rho\}$}
        %\snote{Should the $\cY_i^r$ in this line and the next line be $\cY^{r, \chi}_i$?}}
        	{Let $\Lambda_{r,\chi,t,\rho}(i,*) \triangleq \begin{cases}[(Y', \1[\estreslis(y(X^r_i),Y',\tfrac{1}{t},\tau) > \kappa_t])]_{Y' \in \cY_i^{r,\chi}}, & \left|\cY_i^{r,\chi}\right| \in [0.5,1]\rho \\
        	\emptyset
        	 & \text{otherwise}.\end{cases}$ \\
        	 }
       Let $G_{r,\chi,t,\rho} \triangleq \estgenlis(\Lambda_{r,\chi,t,\rho}, \lambda t) \cdot 0.3 \kappa_t$.\nnote{add tree parameters for trimtree calls to \estgenlis, \estreslis... add genuine element discretization...} \\
       Compute $L_{r,\chi,t,\rho} \gets G_{r,\chi,t,\rho} \circ \Lambda_{r,\chi,t,\rho}$ using Lemma~\ref{lm::tree_decomposition} and $T$.
  		%Let $T_g \gets \textsc{TrimTree}(T,\{(X^r_i,\cY^r_i)\}_i,\kappa_t)$.  \\
    %   Compute $L_{r,t} \gets \genlis(g_{r,t}, \lambda t, T_g) \cdot 0.4 \kappa_t$.
       %}
       }}}
    \Return $\widehat{L} \gets \max_{r,\chi,t,\rho} L_{r,\chi,t,\rho}$.
\end{algorithm}
\caption{Description of the algorithm $\estreslis$.}
\label{fig::ALG_reslis_amended}
\end{figure}

\begin{figure}[h!] 
\setstretch{1.2}
\begin{algorithm}[H]
\caption{\partition}
		\DontPrintSemicolon
		\SetNoFillComment
		\KwIn{Integers $r \in E_2(1/\lambda) \cdot |X|/b$, $\chi \in E_2(k)$ and $i \in [|X|/r]$.} %(assume for now an interval\ns{we expect most blocks LIS to intersect with ``one part'' of $Y$ and in any case should be easily reducible to that})
%and a sequence of $y$-values of length $S^r$.}
		\KwOut{Set of candidate intervals $\cY_i^{r,\chi}$}%\\
	 Let $\cS = \cS^{r,\chi}_i$, and $\cS^p = \cS^{2r,\chi}_{\lceil i/2 \rceil}$.\\
      $\cY \gets \left\{[a,b] \in \cS^p \mid (a,b) \cap \cS = \emptyset \wedge \left([a,b] \cap \cS \neq \emptyset \vee |[a,b) \cap \cS^p| \text{ is power of 2.} \right)\right\}$ \\
	\Return $\cY$.
%\EndFunction
\end{algorithm}
\label{fig::ALG_partition}
\end{figure}


%%%
%
% Stuff from before
%
%%%


%\cdot \log^2 1/\lambda$.
 
     %Let $\cS^r_i \gets (y_{((i-1)r+j)\log n})_{j\in[r]}$
      %, i.e., $X^r_i = [w_{(i-1)r\log n+1}, w_{ir\log n}]$.
          %Let $X^r_1,\ldots,X^r_{b/r}$ be a partition of $X$ into $b/r$ consecutive disjoint intervals each consisting of $r\cdot \log n$ (non-rejected) samples, i.e., $X^r_i = [w_{(i-1)r\log n+1}, w_{ir\log n}]$%\footnote{Note that we do not impose that $X_i$'s have equal width.}  \\
 %    For $i \in [b/r]$, let $\cS^r_i=(y_{((i-1)r+j)\log n})_{j\in[r]}$ be the $y$ values of the $r$ samples in $X^r_i$ whose order is a multiple of $\log n$. \\
     %sorted in descending order; %We assume (by construction) such $\cS^r_i$ are in decreasing order;
   %     Let $g \triangleq Y_{1,1},Y_{1,2},\ldots,Y_{1,r-1},Y_{2,1},\ldots,Y_{b/r,r-1}$ be a $\genlis_b$ input string.  \\   
%\Function{\partition}{$r,i$}
       %\nnote{this is abuse of notation since $\genlis$ is defined on numbers and not intervals. I will see if I can reduce to fixed numbers and if not, will define inputs for both $\genlis$ and $\reslis$ to be of interval spaces to avoid such an issue. in any case dont expect an issue here...} \\
       %\nnote{We first order by $i$ ascending, then by $\cY_i^r$ descending. Note that we use interval input rather than numbers for now. Formalize this better!}\\
  %     Let $\1[\reslis(X_i,Y_{i,j},1/k) > 1/k]$ be the genuine value of each element of $g$. \\
  
%\begin{figure}[t] \label{fig::ALG_partY}
%\setstretch{1.2}
%  \begin{algorithm}[H]
%    \caption{\partition}
%		\DontPrintSemicolon
%		\SetNoFillComment
%		\KwIn{Integers $r \in 2^{[\log (1/\lambda)]}$ and $i \in [b/r]$.} %(assume for now an interval\ns{we expect most blocks LIS to intersect with ``one part'' of $Y$ and in any case should be easily reducible to that})
%%and a sequence of $y$-values of length $S^r$.}
%		\KwOut{An interval sequence $\cY$.}%\\
%		Let $\cS = \cS^r_i$, and $\cS^p = \cS^{2r}_{\lceil i/2 \rceil}$.\\
%     $\cY \gets \left\{[a,b] \in \cS^p \mid (a,b) \cap \cS = \emptyset \wedge \left([a,b] \cap \cS \neq \emptyset \vee |[a,b) \cap \cS^p| \text{ is power of 2.} \right)\right\}$ \\
%	return $\cY$
%\end{algorithm}
%\end{figure}


%\ns{The block size $b$ should be fixed when recursing in genuine tests, but should become smaller when converting the $\genlis$ to $\reslis$... need to write that down...}


==> reslis_inv.tex <==
\subsubsection{Proof of \Cref{lm::reslis_invariants_tree}}\label{sec::resinv_proof}
%\subsubsection{Proof of Lemma~\ref{lm::reslis_invariants}}
%\ns{@Sandip - can you please take care of that?}

%for 4: use 7.3 and show by induction on the radius, divide and conquer on both sides and the overlap interval using the larger radius

\paragraph{Proof of item (1):}

Fix $i,r, \chi$. By construction, we have for all $Y' \in \cY_i^{r, \chi}$ that $Y' \cap \cS_i^{r,\chi} = \emptyset$. In particular, that implies $|p^\chi \cap Y'| < \zeta$. Now fix some $p_i \in p^\chi$ and let $E(p_i)$ be the set of $\tfrac{1.1}{b}|X|\chi$ %\snote{This was $\tfrac{1.1}{b}||X|\chi$}
elements immediately before $p_i$ in $y(X_i^{r,\chi})$. The probability a uniform sample will fall in $E(p)$ is $\tfrac{1.1}{b}\cdot \tfrac{|X|\chi}{|X|\chi} = \tfrac{1.1}{b}$.

Notice that if the number of other sampled points in $E(p_i)$ is at least $\zeta$, then any candidate interval $Y' \subseteq [p_{i-1},p_i]$ %\nnote{define range of elements}
 is of length $\tfrac{1.1}{b}\cdot |X|\chi$.

Overall, we sample $\zeta b - 1$ other elements, and hence the expected number of elements in $E(p_i)$ is $>1.09\zeta$. This quantity is a sum of independent random variables bounded by 1, and hence w.h.p., it will be more than $\zeta$. By union bound over all $p^\chi$ for all $\chi$, we obtain the claim w.h.p. as well. 


\paragraph{Proof of item (2):}%\snote{Items 1 import from next sec, edit notation.}

%\ns{adapt to new setting, mostly just add the sum over $\chi$...}
For $t \in [\tau]$, consider a binary tree $T_t$ of height $\log_2 (1/\lambda)$ where each node represents a $(r,i)$-pair as above. We use $X_v$ for interval $X_i^r$, and similarly $X_v^\chi$ for interval $X_i^{r,\chi}$. For candidate $y$-intervals, we use denote $\cY^\chi_{v}$ for $\cY_i^{r,\chi}$ and $\cY_v \triangleq \cup_\chi \cY^\chi_v$. The leaves $v^1_i$ represent the smallest-size intervals $X_i^1$. For each node $v^r_i$ %represent interval $X^r_{i}$ with 
we connect with the children are $v^{r/2}_{2i-1}$ and $v^{r/2}_{2i}$ as children. Note that each $X_v$ node is a concatenation of $X_{l(v)}$ and $X_{r(v)}$. The roots are $v_t^{1/\lambda}$.


    To define the sets $\widetilde{\cY_i^{r,\chi}}$, we make the following definitions and notations:
    

    
    \begin{definition}
    	Fix a finite set of intervals $S \subseteq \cI$.\footnote{Recall that $\cI = \{[a,b] \mid a,b \in \N: a \leq b \}$ is the set of all possible closed sub-intervals of $\mathbb{N}$.} 
    	The {\em top interval} $\top(S)$ is the interval which contains the maximal value in $\cup_{I \in S} I$ and is not a subset of %contained in\snote{do you mean "not a subset of"?}
    	any other interval in $S$.
    	 Similarly, the {\em bottom interval} $\bot(S)$ is the interval which contains the minimal value in $\cup_{I \in S} I$ and is not a subset of %contained in
    	 any other interval in $S$. 
    \end{definition}
    
   
   Next, for optimal increasing subsequence $y(X^*)$ for $\LIS(X,Y)$, let $M_i^r \triangleq \max\{y(X_i^r \cap X^*)\}$ be the maximal value of $y(X^*)$ in $X_i^r$ (by convention, $M^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_i^r \triangleq (M_{j}^r,M_i^r]$ for the largest $j<i$ such that $M_j^r$ is defined (similarly, let $U^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_v = U_i^r$ for $v=v_i^r$.
   
   We define the following candidate intervals for each $\chi$:
   %containing all $\reslis$ values of $X_v$, i.e.,:
%$$U_v \triangleq [\min y(X^* \cap X_v),\max y(X^* \cap X_v)]$$


    $$\Ytop_{v,\chi} \triangleq %\left\{ Y_{v,j} \mid 
    \top(\{Y \in \cY^\chi_v \mid Y \subseteq U_v\})$$
    
    %} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} < Y_{v,j} \right\}$$

   % $$Y_v^\top \triangleq \left\{ Y_{v,j} \mid 
   % \top(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
   $$\Ybot_{v,\chi} \triangleq %\left\{ Y_{v,j} \mid 
    \bot(\{Y \in \cY^\chi_v \mid Y \subseteq U_v\})$$
    
    %\triangleq \left\{ Y_{v,j} \mid Y_{v,j} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} > Y_{v,j} \right\}$$

    $$\Yplus_{v,\chi} \triangleq %\left\{ Y_{v,j} \mid 
    \top\footnote{$\top$ can be $\bot$ as well, as they are equal for this set.}\left(\left\{Y \in \cY_v^\chi \mid Y \subseteq U_v \wedge \left(U_{l(v)} \setminus Y <  Y\right) \wedge \left(U_{r(v)} \setminus Y > Y\right)  \right\}\right)$$
 

Now for each $v=v_{r,i}$ in the tree, let $\widetilde{\cY^\chi_v}  = \widetilde{\cY_i^{r,\chi}} \triangleq \{\Ytop_{v,\chi},\Ybot_{v,\chi},\Yplus_{v,\chi}\}$. %\{ \top(\{Y \in \cY_v \mid Y \subseteq U_v\}), \bot(\{Y \in \cY_v \mid Y \subseteq U_v\})\}$ .%for even $i$ and $\cY_i^r \triangleq \{Y_v^c,Y_v^o\}$ for odd $i$.

To prove the Lemma, we claim the following:

\begin{claim}\label{cl::coherent_sets}
	For each $r,\chi$, the set $(i,\cup_{Y \in \widetilde{\cY_i^{r,\chi}}} Y)$ is coherent.
\end{claim}

\begin{claim}\label{cl::sum_of_descendants}
 For each $v,\chi$:	
		$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY^\chi_u}}\LIS(X^\chi_u,Y) \geq \LIS(X^\chi_v,\cup_{Y \in \cY^\chi_v: Y \subseteq U_v} Y)$$
\end{claim}

We defer the proofs of Claims \ref{cl::coherent_sets} and \ref{cl::sum_of_descendants}. To complete the argument, % using Claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}
all that is left is to apply Claim~\ref{cl::sum_of_descendants} on the roots, and get the following bound:

\begin{align*}
\LIS(X,Y) &= \sum_i \LIS(X_i^{1/\lambda},U_i^{1/\lambda}) \\
&\leq \sum_i \sum_\chi \LIS(X_i^{1/\lambda,\chi},U_i^{1/\lambda}) \\
 &\leq \sum_i \sum_\chi \left(\LIS(X_i^{1/\lambda, \chi},\cup_{Y' \in \cY_i^{1/\lambda,\chi}: Y' \subseteq U_i^{1/\lambda}} Y') + \LIS(X^{1/\lambda,\chi}_i),U_i^{1/\lambda} \setminus \cup_{Y' \in \cY_i^{1/\lambda,\chi}: Y' \subseteq U_i^{1/\lambda}} Y' \right) \\
  &\leq \sum_i \sum_\chi \left(\LIS(X_i^{1/\lambda,\chi},\cup_{Y' \in \cY_i^{1/\lambda,\chi}: Y' \subseteq U_i^{1/\lambda}} Y') + \tfrac{2}{\chi}\nnote{I think that is wrong! can't divide by $\chi$!}|y(X^{1/\lambda,\chi}_i) \cap U_i^{1/\lambda} \setminus \cup_{Y' \in \cY_i^{1/\lambda,\chi}: Y' \subseteq U_i^{1/\lambda}} Y'| \right)%\snote{Are we assuming all $y$-values are distinct?}
  \\
 &\leq \sum_i \sum_\chi \left(\sum_r \sum_{Y' \in \widetilde{\cY_i^{r,\chi}}}\LIS(X_i^{r,\chi},Y') + 5\lambda  |X_i^{1/\lambda,\chi}|\right)	\\
 &\leq \sum_i \sum_\chi \sum_r \sum_{Y' \in \widetilde{\cY_i^{r,\chi}}}\LIS(X_i^r,Y') + 5\lambda |X|,
\end{align*}

\ns{Problem! can't divide by $\chi$ in line (4)!!}
as needed.
We now prove Claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}.

\begin{proof}[Proof of Claim~\ref{cl::coherent_sets}]
	By definition, we have each $Y \in \widetilde{\cY_i^{r,\chi}}$ is contained in $U_i^r$, hence $\cup_{Y \in \widetilde{\cY_i^{r,\chi}}} Y \subseteq U_i^r$. Now, clearly, for any $r$, the set $\{(i,U_i^r)\}_i$ is coherent, and therefore the set $\{(i,\cup_{Y \in \widetilde{\cY_i^{r,\chi}}} Y )\}_i$  is coherent as well.
\end{proof}

The second claim requires more work.

\begin{proof}[Proof of Claim~\ref{cl::sum_of_descendants}]

For all the below, since $\chi$ is fixed, we dropped the $\chi$ notation from $\cS_v^\chi, \cY_v^\chi$ and so forth and we use $\cS_v, \cY_v$ to denote these sets.

Let $\cS^*_v \triangleq \cS_v \cap U_v$ be the set of sampled coordinates in range. Also let   $p(v)$ denotes the parent of $v$.

	Let $Y_v^* \triangleq \cup_{Y \in \cY_v: Y \subseteq U_v} Y = \left[\min\{\cS^*_{p(v)}\cap U_v\},\max\{\cS^*_{p(v)}\cap U_v\}\right]$. We need to show:
	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,Y_v^*).$$
	
	 We prove by induction on the tree level. For leaves, $|\cY_v|=1$ and hence if such interval is contained in $U_v$, then $\widetilde{\cY_v} = \{Y_v^*\}$.
	
 Now consider the following cases:
	
		\paragraph{There are samples in range:} If $\cS^*_v \neq \emptyset$, then $\Ytop_v = [\max\{\cS^*_v\},\max\{\cS^*_{p(v)}\}]$ and $\Ybot_v = [\min\{\cS^*_{p(v)}\},\min\{\cS^*_v\}]$. This implies 
		$$\LIS(X_v,Y_v^*) \leq \LIS(X_v,\Ytop_v) + \LIS(X_v,\Ybot_v) + \LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\}))$$
		
		The last quantity needs to be broken down further.
		Let $\cSleft_{v} = \cS_v \cap U_{l(v)}$ and $\cSright_{v} = \cS_v \cap U_{r(v)}$. Since $U_{l(v)}$ and $U_{r(v)}$ are consecutive, we have $\cSleft_v \cup \cSright_v = \cS^*_{v}$. %\ns{fix this later by defining the $U_v$ to have no gaps}, 
		Thenn either $\cS_v^* = \cSleft_v$, $\cS_v^* = \cSright_v$ or $\Yplus_v = [\max\{\cSleft_v\},\min\{\cSright_v\}]$. %\aanote{one could be empty}\nnote{fixed} 
		In either case we have overall:
		
			\begin{align*}
			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			&\leq \LIS(X_v,\Yplus_v) \\
			&+\LIS(X_{l(v)},(\min\{\cSleft_v\},\max\{\cSleft_v\}))  \\
			&+\LIS(X_{r(v)},(\min\{\cSright_v\},\max\{\cSright_{v}\}))				
			\end{align*}
			
			%\ns{Check if need to change $\LIS(X_v,Y_v)$ to $|y(X_v \cap X^*)|$ throughout.}
			
			Note that by definition, $Y_{l(v)}^* = [\min\{\cSleft_v)\},\max\{\cSleft_v\}]$ and $Y_{r(v)}^* = [\min\{\cSright_v\},\max\{\cSright_{v}\}]$, hence we get:
		
	$$
			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			\leq \LIS(X_v,\Yplus_v) 
			+\LIS(X_{l(v)},Y_{l(v)}^*)  
			+\LIS(X_{r(v)},Y_{r(v)}^*)				
$$

which by induction can be upper bounded by:
$$
\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
			\leq \LIS(X_v,\Yplus_v) 
			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)$$
			
Hence we conclude 

\begin{align*}
\LIS(X_v,Y_v^*) 
&\leq \LIS(X_v,\Ytop_v) + \LIS(X_v,\Ybot_v) + \LIS(X_v,\Yplus_v) 
			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)\\
		&= \sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)
\end{align*}
			
\paragraph{There are no samples in range:}
Now, consider the case $\cS^*_v = \emptyset$, then we claim $\Ytop_v \cup \Ybot_v = Y_v^*$. Indeed, fix $\cS^*_{p(v)}$, and let
$q$ be the largest exponent of $2$ such that $q \leq |\cS^*_{p(v)}|-1$ (if $|S_{p(v)}^*|=0$ then $Y^*_v=\emptyset$ and there's nothing to prove).\snote{What happens if $|S_{p(v)}^*|$ is 1 ? In that case $q \leq 0$, which doesn't make sense.} Now enumerate $\cS^*_{p(v)} := \{ S_j, S_{j+1},\ldots,S_{j+w} \}$ for some $w < 2q-1$. Then $\Ytop_v = [S_{j+w-q},S_{j+w}]$ and $\Ybot_v = [S_{j},S_{j+q}]$. Overall, $\Ytop_v \cup \Ybot_v = [S_j,S_{j+w}] = Y_v^*$.

We conclude the proof noting:
	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,\Ytop_v) + \LIS(X_v,\Ybot_v) \geq \LIS(X_v,Y_v^*).$$
	

\end{proof}






%%%
%
% Old stuff
%
%%%


%\subsection{Old - Invariants proof (1-3)}
%
%\ns{see if we need anything from below and integrate with new invariants...}
%We will use the following tail bounds for sums of independent geometric random variables, which are special cases of results proved by~\cite{Janson18}.
%\begin{theorem}[Theorems 2.1 and 3.1 in~\cite{Janson18}] \label{thm:janson_geometric_tail}
%	Let $p \in (0,1]$, and $\bX_1,\cdots, \bX_m$ be independent \emph{Geometric}\hspace{0.04cm}$(p)$ random variables. Let $\bX = \sum_{i\in [m]} \bX_i$ and $\mu = \bE[\bX] = m/p$. Then for any $\alpha \in (0,1)$, we have 
%	\[
%		\Pr\big[X \notin [(1-\alpha)\mu, (1 +\alpha)\mu]\big] \leq 2 \exp\left({-p \mu (\alpha - \ln (1+\alpha)}\right).
%	\]
%\end{theorem}
%Note that $\alpha - \ln (1+\alpha) \geq 0$ for all $\alpha \in (0,1)$, with equality only at $\alpha = 0$. We first derive a simpler expression for the tail bounds, using the following claim:
%\begin{claim} \label{clm:Janson_simple}
%	Let $f : (-1,\infty) \rightarrow \R$ be defined as
%	$
%	f(x) = x - \ln (1+x).
%	$
%	The following  properties hold:
%(i) $f(0) = 0$; (ii) $f(x) > x^2/4$ for all $x \in (-1,1]  \setminus \{0\}$; and
%(iii) $f(x) \geq x/4$ for all $x \geq 1$.\snote{Note to self: Probably don't need the third property; check and remove.}
%\end{claim}
%\begin{proof}
%	The claim follows from elementary calculus. For item (ii) it can be shown that  $g(x) = f(x) - x^2/4$ attains its minimum value $0$ at $x = 0$ and is strictly convex in $(-1,1]$. For item (iii) it is easy to verify that $h(x) = f(x) - x/4$ satisfies $h'(x) > 0$ for all $x \geq 1$, and hence its minimum value is $h(1) \geq 0.05$.
%\end{proof}
%%Letting $x = \lambda - 1$ in~\Cref{thm:janson_geometric_tail}, this claim allows us to replace the $\lambda - 1 - \ln \lambda$ term in the exponent of the tail bounds by either $(\lambda-1)^2 / 4$ or $(\lambda-1)/4$, depending on whether $\lambda < 2$ or $\lambda \geq 2$.
%
%
%\begin{proofof}{\Cref{lm::reslis_invariants_new}}
%\ns{see what we need here and integrate into new invariants once done..}
%We now prove each invariant stated in the lemma.\snote{Note to self: Change $X \cap Y^{-1}$ to $y(X) \cap Y$ everywhere.}
%\begin{enumerate}
%    \item Each element of $X \cap Y^{-1}$ is sampled with probability
%    \[
%    p := \frac{b \log n}{|X \cap Y^{-1}|}.
%    \]
%    Fix a node $v \in V$, and let $r_v$ be the corresponding interval length. Then, we observe that $|X_v \cap Y^{-1}|$ is a sum of $r_v \log n$ independent Geometric$(p)$ random variables.\snote{Does this require more explanation?} So, we have
%    \[
%        \mu := \E\left[\left|X_v \cap Y^{-1}\right|\right] = \frac{r_v \log n}{p} = \frac{r_v}{b} \left|X \cap Y^{-1}\right|.
%    \]
%    Now, applying \Cref{thm:janson_geometric_tail} with $p,\mu$ as above and $\alpha = 0.1$, we have
%    \[
%        \Pr\left[\left|X_v \cap Y^{-1}\right| \notin \left[\frac{0.9 r_v}{b} \left|X \cap Y^{-1}\right|, \frac{1.1 r_v}{b}\left|X \cap Y^{-1}\right|\right]\right] \leq \exp(-\Omega(p \mu)) = \exp(-\Omega(r_v \log n)) \leq \frac{1}{n^3},
%    \]
%    by choosing a sufficiently large constant in the  sampling rate.\snote{Make sure the algorithm does this.} Using a union bound over all $v \in V$, we conclude that Item (1) holds with probability at least $1-1/n^2$. We assume that this invariant holds for the rest of the proof.
%    
%    \item Each element in $X_v \cap Y{-1}$ is sampled with probability
%    \[
%        p':= \frac{r \log n}{|X_v \cap Y^{-1}|}.
%    \]
%    For for each $j \in [r-1]$, $|X_v \cap Y_{v,j}^{-1}|$ \blue{(equivalently, $|y(X_v) \cap Y_{v,j}|$)}\snote{Only holds if all elements distinct} is a sum of $\log n$ independent Geometric($p'$) random variables. So,
%    \[
%        \mu':= \E\left[\left|X_v \cap Y_{v,j}^{-1}\right|\right] = \frac{\log n}{p'} = \frac{|X_v \cap Y^{-1}|}{r_v} \in \left[\frac{0.9}{b} \left|X \cap Y^{-1}\right|, \frac{1.1}{b} \left|X \cap Y^{-1}\right|\right],
%    \]
%    where we have used the previous invariant to bound $\mu'$. Again we invoke \Cref{thm:janson_geometric_tail} with $p',\mu'$ as above and $\alpha = 0.1$ to get that with probability at least $1-1/n^3$,
%    \[
%    \left|X_v \cap Y_{v,j}^{-1}\right| \in [0.9\mu', 1.1\mu'] \subset \left[\frac{0.81}{b} \left|X \cap Y^{-1}\right|, \frac{1.21}{b}\left|X \cap Y^{-1}\right|\right].
%    \]
%    
%    \item %\snote{This is proof of \Cref{lm::reslis_invariants}, item 3; need to edit notation and paste there.}
%    Fix $r \in 2^{[\log (1/\lambda)]}$. Consider a coherent set $\{(i,Y^r_{i,j(i)}\}_{i \in [b/r]}$, where for each $i \in [b/r]$, there is at most one $j=j(i)\in [r-1]$ such that $Y^r_{i,j(i)}$ is part of the set. \snote{The lemma statement needs to specify that $j$ is a function of $i$.}
%    Then by definition of a coherent set and the order relation over intervals, we have $i_1 < i_2 \equiv \max(Y^r_{i_1,j(i_1)}) < \min(Y^r_{i_2,j(i_2)})$. For each $i \in [b/r]$, let $\cL_i$ be the longest increasing sequence in $X_i$\footnote{We choose one sequence arbitrarily if there are multiple longest increasing sequences.}, with values restricted to $Y^r_{i,j(i)}$. $\LIS(X_i, Y^r_{i,j(i)})$. By the property of coherence and the fact that $Y^r_{i,j(i)}) \subset Y$ for all $i$, the sequence $\cL = \cup_i \cL_i$ is clearly a valid increasing subsequence of $X$ with values restricted to $Y$. As this subsequence has length $\sum_i \LIS(X_i, Y^r_{i,j(i)})$, we conclude that $\sum_i \LIS(X_i, Y^r_{i,j(i)}) \leq \LIS(X,Y)$.
%    
%\end{enumerate}
%    
%\end{proofof}


%%%
%
% OLD PROOF
%
%%%


%
%For $t \in [n^\eps]$, Consider a binary tree $T_t$ of height $\log_2 1/\lambda$ where each node represent a $(r,i)$-pair as above. We use $X_v$ for interval $X_i^r$ and $\cY_{v,j}$ for candidate $y$-intervals. The leaves $v^1_i$ represent the smallest-size intervals $X_i^1$. For each node $v^r_i$ %represent interval $X^r_{i}$ with 
%we connect with the children are $v^{r/2}_{2i-1}$ and $v^{r/2}_{2i}$ as children. Note that each $X_v$ node is a concatenation of $X_{l(v)}$ and $X_{r(v)}$. The roots are $v_t^{1/\lambda}$.
%
%
%
%    To define the sets $\widetilde{\cY_i^r}$ we make the following definitions and notations:
%    
%
%    
%    \begin{definition}
%    	Fix a finite set of intervals $S \subseteq \cI$. 
%    	The {\em top interval} $\top(S)$ is the interval which contains the maximal value in $\cup_{I \in S} I$ and is not contained in any other interval in $S$.
%    	 Similarly, the {\em bottom interval} $\bot(S)$ is the interval which contains the minimal value in $\cup_{I \in S} I$ and is not contained in any other interval in $S$. 
%    \end{definition}
%    
%   
%   Next, for optimal increasing subsequence $y(X^*)$ for $\LIS(X,Y)$, let $M_i^r \triangleq \max\{y(X_i^r \cap X^*)\}$ be the maximal value of $y(X^*)$ in $X_i^r$ (by convention, $M^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_i^r \triangleq (M_{j}^r,M_i^r]$ for the largest $j<i$ such that $M_j$ is defined (similarly, let $U^r_i = \bot$ if $X^* \cap X_i^r = \emptyset$). Let $U_v = U_i^r$ for $v=v_i^r$.
%   
%   We define the following candidate intervals:
%   %containing all $\reslis$ values of $X_v$, i.e.,:
%%$$U_v \triangleq [\min y(X^* \cap X_v),\max y(X^* \cap X_v)]$$
%
%
%    $$Y_v^\top \triangleq %\left\{ Y_{v,j} \mid 
%    \top(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
%    
%    %} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} < Y_{v,j} \right\}$$
%
%   % $$Y_v^\top \triangleq \left\{ Y_{v,j} \mid 
%   % \top(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
%   $$Y_v^\bot \triangleq %\left\{ Y_{v,j} \mid 
%    \bot(\{Y \in \cY_v \mid Y \subseteq U_v\})$$
%    
%    %\triangleq \left\{ Y_{v,j} \mid Y_{v,j} \subseteq U_{p(v)} \wedge U_v \setminus Y_{v,j} > Y_{v,j} \right\}$$
%
%    $$Y_v^+ \triangleq %\left\{ Y_{v,j} \mid 
%    \top\nnote{$\top$ can be $\bot$ as well, as they are equal for this set.}\left(\left\{Y \in \cY_v \mid Y \subseteq U_v \wedge \left(U_{l(v)} \setminus Y <  Y\right) \wedge \left(U_{r(v)} \setminus Y > Y\right)  \right\}\right)$$
% 
%
%Now for each $v=v_{r,i}$ in the tree, let $\widetilde{\cY_v}  = \widetilde{\cY_i^r} \triangleq \{Y_v^\top,Y_v^\bot,Y_v^+\}$. %\{ \top(\{Y \in \cY_v \mid Y \subseteq U_v\}), \bot(\{Y \in \cY_v \mid Y \subseteq U_v\})\}$ .%for even $i$ and $\cY_i^r \triangleq \{Y_v^c,Y_v^o\}$ for odd $i$.
%
%To prove the Lemma, we claim the following:
%
%\begin{claim}\label{cl::coherent_sets}
%	For each $r$, the set $(i,\cup_{Y \in \widetilde{\cY_i^r}} Y)$ is coherent.
%\end{claim}
%\begin{claim}\label{cl::sum_of_descendants}
% For each $v$:	
%		$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,\cup_{Y \in \cY_v: Y \subseteq U_v} Y)$$
%\end{claim}
%
%To complete the argument, % using Claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}
%all that is left is to apply Claim~\ref{cl::sum_of_descendants} on the roots, and get the following bound:
%
%\begin{align*}
%\LIS(X,Y) &= \sum_i \LIS(X_i^{1/\lambda},U_i^{1/\lambda}) \\
% &\leq \sum_i \left(\LIS(X_i^{1/\lambda},\cup_{Y' \in \cY_i^{1/\lambda}: Y' \subseteq U_i^{1/\lambda}} Y') + |y(X_i) \cap U_i^{1/\lambda} \setminus \cup_{Y' \in \cY_i^{1/\lambda}: Y' \subseteq U_i^{1/\lambda}} Y'| \right) \\
% &\leq \sum_i \left(\sum_r \sum_{Y' \in \widetilde{\cY_i^r}}\LIS(X_i^r,Y') + 2.2\lambda  |y(X_i) \cap Y|\right)	\\
% &\leq \sum_i \sum_r \sum_{Y' \in \widetilde{\cY_i^r}}\LIS(X_i^r,Y') + 2.2\lambda  |y \cap Y|	
%\end{align*}
%
%as needed.
%
%We now prove claims~\ref{cl::coherent_sets} and~\ref{cl::sum_of_descendants}.
%
%\begin{proof}[Proof of Claim~\ref{cl::coherent_sets}]
%	By definition, we have each $Y \in \widetilde{\cY_i^r}$ is contained in $U_i^r$, hence $\cup_{Y \in \widetilde{\cY_i^r}} Y \subseteq U_i^r$. Now, clearly, for any $r$, the set $\{(i,U_i^r)\}_i$ is coherent, and therefore the set $\{(i,\cup_{Y \in \widetilde{\cY_i^r}} Y )\}_i$  is coherent as well.
%\end{proof}
%
%The second claim requires more work.
%
%\begin{proof}[Proof of Claim~\ref{cl::sum_of_descendants}]
%Let $\cS^*_v \triangleq \cS_v \cap U_v$ be the set of sampled coordinates in range. Also let   $p(v)$ denotes the parent of $v$.
%
%	Let $Y_v^* \triangleq \cup_{Y \in \cY_v: Y \subseteq U_v} Y = \left[\min\{\cS^*_{p(v)}\cap U_v\},\max\{\cS^*_{p(v)}\cap U_v\}\right]$. We need to show:
%	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,Y_v^*).$$
%	
%	 We prove by induction on the tree level. For leaves, $|\cY_v|=1$ and hence if such interval is contained in $U_v$, then $\widetilde{\cY_v} = \{Y_v^*\}$.
%	
% Now consider the following cases:
%	
%		\paragraph{There are samples in range:} If $\cS^*_v \neq \emptyset$, then $Y_v^\top = [\max\{\cS^*_v\},\max\{\cS^*_{p(v)}\}]$ and $Y_v^\bot = [\min\{\cS^*_{p(v)}\},\min\{\cS^*_v\}]$. This implies 
%		$$\LIS(X_v,Y_v^*) \leq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) + \LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\}))$$
%		
%		The last quantity needs to be broken down further.
%		Let $\cSleft_{v} = \cS_v \cap U_{l(v)}$ and $\cSright_{v} = \cS_v \cap U_{r(v)}$. Since $U_{l(v)}$ and $U_{r(v)}$ are consecutive, we have $\cSleft_v \cup \cSright_v = \cS^*_{v}$. %\ns{fix this later by defining the $U_v$ to have no gaps}, 
%		Therefore $Y_v^+ = [\max\{\cSleft_v\},\min\{\cSright_v\}]$. \aanote{one could be empty}\nnote{then we set $Y_v^+=\emptyset$, i.e., we dont need it... } Overall:
%		
%			\begin{align*}
%			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
%			&\leq \LIS(X_v,Y_v^+) \\
%			&+\LIS(X_{l(v)},(\min\{\cSleft_v\},\max\{\cSleft_v\}))  \\
%			&+\LIS(X_{r(v)},(\min\{\cSright_v\},\max\{\cSright_{v}\}))				
%			\end{align*}
%			
%			\ns{Check if need to change $\LIS(X_v,Y_v)$ to $|y(X_v \cap X^*)|$ throughout.}
%			
%			Note that by definition, $Y_{l(v)}^* = [\min\{\cSleft_v)\},\max\{\cSleft_v\}]$ and $Y_{r(v)}^* = [\min\{\cSright_v\},\max\{\cSright_{v}\}]$, hence we get:
%		
%	$$
%			\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
%			\leq \LIS(X_v,Y_v^+) 
%			+\LIS(X_{l(v)},Y_{l(v)}^*)  
%			+\LIS(X_{r(v)},Y_{r(v)}^*)				
%$$
%
%which by induction can be upper bounded by:
%$$
%\LIS(X_v,(\min\{\cS^*_v\},\max\{\cS^*_v\})) 
%			\leq \LIS(X_v,Y_v^+) 
%			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)$$
%			
%Hence we conclude 
%
%\begin{align*}
%\LIS(X_v,Y_v^*) 
%&\leq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) + \LIS(X_v,Y_v^+) 
%			+ \sum_{u \text{ is descendant of } l(v) \text{ or } r(v)} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)\\
%		&= \sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y)
%\end{align*}
%			
%\paragraph{There are no samples in range:}
%Now, consider the case $\cS^*_v = \emptyset$, then we claim $Y_v^\top \cup Y_v^\bot = Y_v^*$. Indeed, fix $\cS^*_{p(v)}$, and let
%$q$ be the largest exponent of $2$ such that $q \leq |\cS^*_{p(v)}|-1$ (if $|S_{p(v)}^*|=0$ then $Y^*_v=\emptyset$ and there's nothing to prove). Now enumerate $\cS^*_{p(v)} := \{ S_j, S_{j+1},\ldots,S_{j+w} \}$ for some $w < 2q-1$. Then $Y_v^\top = [S_{j+w-q},S_{j+w}]$ and $Y_v^\bot = [S_{j},S_{j+q}]$. Overall, $Y_v^\top \cup Y_v^\bot = [S_j,S_{j+w}] = Y_v^*$.
%
%We conclude the proof noting:
%	$$\sum_{u \text{ is descendant of } v} \sum_{Y \in \widetilde{\cY_u}}\LIS(X_u,Y) \geq \LIS(X_v,Y_v^\top) + \LIS(X_v,Y_v^\bot) \geq \LIS(X_v,Y_v^*).$$
%	
%
%\end{proof}
%
%\subsection{Old - Invariants proof (1-3)}
%
%\ns{see if we need anything from below and integrate with new invariants...}
%We will use the following tail bounds for sums of independent geometric random variables, which are special cases of results proved by~\cite{Janson18}.
%\begin{theorem}[Theorems 2.1 and 3.1 in~\cite{Janson18}] \label{thm:janson_geometric_tail}
%	Let $p \in (0,1]$, and $\bX_1,\cdots, \bX_m$ be independent \emph{Geometric}\hspace{0.04cm}$(p)$ random variables. Let $\bX = \sum_{i\in [m]} \bX_i$ and $\mu = \bE[\bX] = m/p$. Then for any $\alpha \in (0,1)$, we have 
%	\[
%		\Pr\big[X \notin [(1-\alpha)\mu, (1 +\alpha)\mu]\big] \leq 2 \exp\left({-p \mu (\alpha - \ln (1+\alpha)}\right).
%	\]
%\end{theorem}
%Note that $\alpha - \ln (1+\alpha) \geq 0$ for all $\alpha \in (0,1)$, with equality only at $\alpha = 0$. We first derive a simpler expression for the tail bounds, using the following claim:
%\begin{claim} \label{clm:Janson_simple}
%	Let $f : (-1,\infty) \rightarrow \R$ be defined as
%	$
%	f(x) = x - \ln (1+x).
%	$
%	The following  properties hold:
%(i) $f(0) = 0$; (ii) $f(x) > x^2/4$ for all $x \in (-1,1]  \setminus \{0\}$; and
%(iii) $f(x) \geq x/4$ for all $x \geq 1$.\snote{Note to self: Probably don't need the third property; check and remove.}
%\end{claim}
%\begin{proof}
%	The claim follows from elementary calculus. For item (ii) it can be shown that  $g(x) = f(x) - x^2/4$ attains its minimum value $0$ at $x = 0$ and is strictly convex in $(-1,1]$. For item (iii) it is easy to verify that $h(x) = f(x) - x/4$ satisfies $h'(x) > 0$ for all $x \geq 1$, and hence its minimum value is $h(1) \geq 0.05$.
%\end{proof}
%%Letting $x = \lambda - 1$ in~\Cref{thm:janson_geometric_tail}, this claim allows us to replace the $\lambda - 1 - \ln \lambda$ term in the exponent of the tail bounds by either $(\lambda-1)^2 / 4$ or $(\lambda-1)/4$, depending on whether $\lambda < 2$ or $\lambda \geq 2$.
%
%
%\begin{proofof}{\Cref{lm::reslis_invariants_new}}
%\ns{see what we need here and integrate into new invariants once done..}
%We now prove each invariant stated in the lemma.\snote{Note to self: Change $X \cap Y^{-1}$ to $y(X) \cap Y$ everywhere.}
%\begin{enumerate}
%    \item Each element of $X \cap Y^{-1}$ is sampled with probability
%    \[
%    p := \frac{b \log n}{|X \cap Y^{-1}|}.
%    \]
%    Fix a node $v \in V$, and let $r_v$ be the corresponding interval length. Then, we observe that $|X_v \cap Y^{-1}|$ is a sum of $r_v \log n$ independent Geometric$(p)$ random variables.\snote{Does this require more explanation?} So, we have
%    \[
%        \mu := \E\left[\left|X_v \cap Y^{-1}\right|\right] = \frac{r_v \log n}{p} = \frac{r_v}{b} \left|X \cap Y^{-1}\right|.
%    \]
%    Now, applying \Cref{thm:janson_geometric_tail} with $p,\mu$ as above and $\alpha = 0.1$, we have
%    \[
%        \Pr\left[\left|X_v \cap Y^{-1}\right| \notin \left[\frac{0.9 r_v}{b} \left|X \cap Y^{-1}\right|, \frac{1.1 r_v}{b}\left|X \cap Y^{-1}\right|\right]\right] \leq \exp(-\Omega(p \mu)) = \exp(-\Omega(r_v \log n)) \leq \frac{1}{n^3},
%    \]
%    by choosing a sufficiently large constant in the  sampling rate.\snote{Make sure the algorithm does this.} Using a union bound over all $v \in V$, we conclude that Item (1) holds with probability at least $1-1/n^2$. We assume that this invariant holds for the rest of the proof.
%    
%    \item Each element in $X_v \cap Y{-1}$ is sampled with probability
%    \[
%        p':= \frac{r \log n}{|X_v \cap Y^{-1}|}.
%    \]
%    For for each $j \in [r-1]$, $|X_v \cap Y_{v,j}^{-1}|$ \blue{(equivalently, $|y(X_v) \cap Y_{v,j}|$)}\snote{Only holds if all elements distinct} is a sum of $\log n$ independent Geometric($p'$) random variables. So,
%    \[
%        \mu':= \E\left[\left|X_v \cap Y_{v,j}^{-1}\right|\right] = \frac{\log n}{p'} = \frac{|X_v \cap Y^{-1}|}{r_v} \in \left[\frac{0.9}{b} \left|X \cap Y^{-1}\right|, \frac{1.1}{b} \left|X \cap Y^{-1}\right|\right],
%    \]
%    where we have used the previous invariant to bound $\mu'$. Again we invoke \Cref{thm:janson_geometric_tail} with $p',\mu'$ as above and $\alpha = 0.1$ to get that with probability at least $1-1/n^3$,
%    \[
%    \left|X_v \cap Y_{v,j}^{-1}\right| \in [0.9\mu', 1.1\mu'] \subset \left[\frac{0.81}{b} \left|X \cap Y^{-1}\right|, \frac{1.21}{b}\left|X \cap Y^{-1}\right|\right].
%    \]
%    
%    \item %\snote{This is proof of \Cref{lm::reslis_invariants}, item 3; need to edit notation and paste there.}
%    Fix $r \in 2^{[\log (1/\lambda)]}$. Consider a coherent set $\{(i,Y^r_{i,j(i)}\}_{i \in [b/r]}$, where for each $i \in [b/r]$, there is at most one $j=j(i)\in [r-1]$ such that $Y^r_{i,j(i)}$ is part of the set. \snote{The lemma statement needs to specify that $j$ is a function of $i$.}
%    Then by definition of a coherent set and the order relation over intervals, we have $i_1 < i_2 \equiv \max(Y^r_{i_1,j(i_1)}) < \min(Y^r_{i_2,j(i_2)})$. For each $i \in [b/r]$, let $\cL_i$ be the longest increasing sequence in $X_i$\footnote{We choose one sequence arbitrarily if there are multiple longest increasing sequences.}, with values restricted to $Y^r_{i,j(i)}$. $\LIS(X_i, Y^r_{i,j(i)})$. By the property of coherence and the fact that $Y^r_{i,j(i)}) \subset Y$ for all $i$, the sequence $\cL = \cup_i \cL_i$ is clearly a valid increasing subsequence of $X$ with values restricted to $Y$. As this subsequence has length $\sum_i \LIS(X_i, Y^r_{i,j(i)})$, we conclude that $\sum_i \LIS(X_i, Y^r_{i,j(i)}) \leq \LIS(X,Y)$.
%    
%\end{enumerate}
%    
%\end{proofof}


==> technical_main.tex <==
%\section{Main Algorithm for Estimating $\LIS$} \label{sec:technical:main}

%\ns{this section should eventually replace section 4 I think...}
%\snote{This section was too big; I split it into 3 sections - the first one is the main technical section which includes the statement of \Cref{thm::gl_rec_tree}, \Cref{thm::sl_rec_tree}, and the proof of \Cref{thm::lis_main} assuming these 2. The second section is about \genlis, and the third is about \reslis.}




%%%
%
% OLD STUFF
%
%%%

% Again, parameter $k$ provides the additional promise that each $k$-coordinate block can contributes at most 1 (genuine) $\LIS$-element. %(we define $m \triangleq |y \cap Y|$).

%We now define pseudo-random oracle:
%
%\begin{definition}
%	Fix $n$ elements $e_1,\ldots,e_n$ that are partitioned to $n/k$ consecutive blocks $B_1,\ldots,B_{n/k}$ of  $k$ elements each. Fix a condition $\cC$ and $\delta \in [0,1]$. A pseudo-random oracle $\cD_{\cC,\delta,k}$ is an oracle that subsamples each block with probability $\delta$, and for each subsampled $B_i$, outputs a uniformly random element $e \in B_i$ that satisfies $\cC$, if such exists.
%\end{definition}
%
%\begin{definition}
%	Fix $n$ elements $\{(X_i,Y_{i,j})\}_{i \in [n/k], j \in [k]}$. A comprehensive pseudo-random oracle $\cD_{\alpha,\lambda,n,k}$ can answer $\cD_{\cC_{\lambda'},\lambda'',k}$ queries wherever:
%	\begin{itemize}
%		\item $\cC_{\lambda'} = \1[\widehat{L}(X_i,Y_{i,j}) > \lambda' |X_i|]$ where $\widehat{L}(X',Y')$ is an $(\alpha,\lambda' |X'|)$-approximation for $\LIS_k(X',Y')$. 
%		\item $\lambda' \cdot \lambda'' \geq \lambda \cdot \log(1/\lambda)$
%	\end{itemize}
%\end{definition}



%\begin{theorem}[$\reslis$ recursive hypothesis - using sample bank]\label{thm::sl_rec}
%% Fix $v \in V_l$ (ie, a node at level $l$). 
%Fix a tree level $l$. Suppose, for some fixed functions $a_g$ and $a_s$ on $\R \rightarrow \R$, there exists algorithms $\cA_{GL}$ that $(a_g(\lambda_g),\lambda_g n_g)$-approximates $\genlis_{n_g}$ using $c_g(\lambda_g)$ complexity\nnote{this part needs to be changed / defined, but not so simple to define atm, needs to start writing the proof first to see exactly how to define},
%	 and $A_{SL}$ that $\left(a_s\left(\tfrac{\Pn_u |X'|}{|y(X') \cap Y'|}\right),\Pn_u |X_u|\right)$-approximates $\LIS(X',Y')$ using $\cB(X_u)$ for any $u \in V_{<l}$ (ie, a node at level $<l$) and $(X', Y') \subseteq X_u \times \N$.
%	 Then, for any $v \in V_l$ and any $(X', Y') \subseteq X_v \times \N$ we can produce a $(\alpha_v, \Pn_v |X_v|)$-approximation for $\LIS(X',Y')$ for any $(X',Y') \subseteq X_v \times \N$, 
%	 where %$n= n_g n_s$, 
%	$\alpha_v = \polylog (1/\Pn_v) \cdot a_s\left(\tfrac{\Pn_v |X'|}{|y(X') \cap Y'|}\right)$ using $\cB(X_v)$.
%\end{theorem}


